The AGN contribution to the UV-FIR luminosities of interacting galaxies and its role in identifying the Main Sequence

Emission from active galactic nuclei (AGNs) is known to play an important role in the evolution of many galaxies including luminous and ultraluminous systems (U/LIRGs), as well as merging systems. However, the extent, duration, and exact effects of its influence are still imperfectly understood. To assess the impact of AGNs on interacting systems, we present a Spectral Energy Distribution (SED) analysis of a sample of 189 nearby galaxies. We gather and systematically re-reduce archival broad-band imaging mosaics from the ultraviolet to the far-infrared using data from GALEX, SDSS, 2MASS, IRAS, WISE, Spitzer and Herschel. We use spectroscopy from Spitzer/IRS to obtain fluxes from fine-structure lines that trace star formation and AGN activity. Utilizing the SED modelling and fitting tool CIGALE, we derive the physical conditions of the ISM, both in star-forming regions and in nuclear regions dominated by the AGN in these galaxies. We investigate how the star formation rates (SFRs) and the fractional AGN contributions ($f_{\rm{AGN}}$) depend on stellar mass, galaxy type, and merger stage. We find that luminous galaxies more massive than about $10^{10} \rm{M}_{*}$ are likely to deviate significantly from the conventional galaxy main-sequence relation. Interestingly, infrared AGN luminosity and stellar mass in this set of objects are much tighter than SFR and stellar mass. We find that buried AGNs may occupy a locus between bright starbursts and pure AGNs in the $f_{\rm{AGN}}$-[Ne V]/[Ne II] plane. We identify a modest correlation between $f_{\rm{AGN}}$ and mergers in their later stages.

==> QuantifiyingAGN_arXiv 2/PhotoTables/2MASS_sigs_stub.tex <==
\begin{tabular}{cccccccc}
\hline
Galaxy & \multicolumn{3}{c}{2MASS} & \multicolumn{4}{c}{{\sl Spitzer}/IRAC} \\
ID     & $J$ & $H$ & $K_s$ & 3.6\,$\mu$m & 4.5\,$\mu$m & 5.8\,$\mu$m & 8.0\,$\mu$m \\
       & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) \\
\hline
\multicolumn{7}{c}{Photometry for the SIGS sample} \\
\hline
NGC274 & 111.29 $\pm$ 2.28 & 132.95 $\pm$ 2.76 & 102.24 $\pm$ 2.28 & 50.25 $\pm$ 1.51 & 31.65 $\pm$ 0.95 & 23.19 $\pm$ 0.70 & 17.06 $\pm$ 0.52 \\
NGC275 & 64.31 $\pm$ 1.41 & 73.18 $\pm$ 1.68 & 59.58 $\pm$ 1.68 & 39.06 $\pm$ 1.17 & 27.29 $\pm$ 0.82 & 70.69 $\pm$ 2.13 & 170.52 $\pm$ 5.12 \\
NGC470 & 186.08 $\pm$ 3.96 & 199.56 $\pm$ 4.58 & 184.86 $\pm$ 4.47 & 108.22 $\pm$ 3.25 & 73.47 $\pm$ 2.20 & 163.96 $\pm$ 4.93 & 417.70 $\pm$ 12.53 \\
NGC474 & 296.05 $\pm$ 7.02 & 314.31 $\pm$ 8.98 & 271.30 $\pm$ 8.35 & 149.83 $\pm$ 4.50 & 86.50 $\pm$ 2.60 & 141.57 $\pm$ 4.34 & 100.29 $\pm$ 3.14 \\
NGC520 & 288.70 $\pm$ 6.23 & 357.34 $\pm$ 8.33 & 312.68 $\pm$ 7.30 & 182.73 $\pm$ 5.48 & 138.65 $\pm$ 4.16 & 357.79 $\pm$ 10.74 & 916.85 $\pm$ 27.51 \\
IC195 & 54.38 $\pm$ 1.22 & 66.50 $\pm$ 1.60 & 53.22 $\pm$ 1.47 & 25.29 $\pm$ 0.76 & 15.80 $\pm$ 0.47 & 10.82 $\pm$ 0.34 & 6.30 $\pm$ 0.21 \\
IC196 & 95.34 $\pm$ 2.39 & 129.52 $\pm$ 3.48 & 105.90 $\pm$ 3.34 & 49.53 $\pm$ 1.49 & 32.17 $\pm$ 0.97 & 29.94 $\pm$ 0.92 & 42.85 $\pm$ 1.30 \\
NGC833 & 101.56 $\pm$ 2.08 & 125.16 $\pm$ 2.62 & 106.44 $\pm$ 2.32 & 48.47 $\pm$ 1.45 & 30.78 $\pm$ 0.92 & 25.01 $\pm$ 0.76 & 25.52 $\pm$ 0.77 \\
NGC835 & 155.86 $\pm$ 3.17 & 194.36 $\pm$ 4.01 & 166.35 $\pm$ 3.51 & 89.23 $\pm$ 2.68 & 60.95 $\pm$ 1.83 & 117.65 $\pm$ 3.53 & 291.88 $\pm$ 8.76 \\
NGC838 & 73.96 $\pm$ 1.57 & 93.24 $\pm$ 2.04 & 86.14 $\pm$ 1.97 & 67.69 $\pm$ 2.03 & 50.08 $\pm$ 1.50 & 212.29 $\pm$ 6.37 & 589.03 $\pm$ 17.67 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/PhotoTables/GALEX_sigs_stub.tex <==
\begin{tabular}{cccccccc}
\hline
Galaxy & \multicolumn{2}{c}{\sl GALEX} & \multicolumn{5}{c}{SDSS DR12} \\
ID     & FUV & NUV & $u$ & $g$ & $r$ & $i$ & $z$ \\
       & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) \\
\hline  
\multicolumn{7}{c}{Photometry for the SIGS sample} \\
\hline
NGC274 & $\cdots$ & $\cdots$ & 4.53 $\pm$ 0.13 & 21.15 $\pm$ 0.42 & 43.97 $\pm$ 0.88 & 64.74 $\pm$ 1.30 & 81.14 $\pm$ 1.66 \\
NGC275 & 3.30 $\pm$ 0.33 & 4.56 $\pm$ 0.46 & 10.80 $\pm$ 0.24 & 23.35 $\pm$ 0.47 & 36.91 $\pm$ 0.74 & 43.79 $\pm$ 0.88 & 50.87 $\pm$ 1.08 \\
NGC470 & 3.18 $\pm$ 0.32 & 4.67 $\pm$ 0.47 & 16.59 $\pm$ 0.37 & 44.43 $\pm$ 0.89 & 78.42 $\pm$ 1.57 & 107.23 $\pm$ 2.15 & 131.44 $\pm$ 2.67 \\
NGC474 & 1.44 $\pm$ 0.15 & 1.98 $\pm$ 0.20 & 20.66 $\pm$ 0.61 & 67.87 $\pm$ 1.36 & 125.69 $\pm$ 2.52 & 179.48 $\pm$ 3.61 & 243.94 $\pm$ 5.05 \\
NGC520 & 1.69 $\pm$ 0.17 & 3.12 $\pm$ 0.31 & 4.25 $\pm$ 0.22 & 62.00 $\pm$ 1.25 & 113.32 $\pm$ 2.27 & 160.68 $\pm$ 3.22 & 192.31 $\pm$ 3.92 \\
IC195 & 0.05 $\pm$ 0.01 & 0.10 $\pm$ 0.01 & 1.96 $\pm$ 0.06 & 9.48 $\pm$ 0.19 & 19.99 $\pm$ 0.40 & 29.45 $\pm$ 0.59 & 37.98 $\pm$ 0.77 \\
IC196 & 0.65 $\pm$ 0.06 & 0.82 $\pm$ 0.08 & 4.33 $\pm$ 0.14 & 18.03 $\pm$ 0.36 & 36.51 $\pm$ 0.73 & 53.72 $\pm$ 1.08 & 68.04 $\pm$ 1.41 \\
NGC833 & $\cdots$ & 0.29 $\pm$ 0.03 & 3.33 $\pm$ 0.09 & 16.49 $\pm$ 0.33 & 35.86 $\pm$ 0.72 & 53.35 $\pm$ 1.07 & 68.14 $\pm$ 1.39 \\
NGC835 & $\cdots$ & 1.67 $\pm$ 0.17 & 7.74 $\pm$ 0.17 & 29.07 $\pm$ 0.58 & 57.24 $\pm$ 1.15 & 81.33 $\pm$ 1.63 & 102.36 $\pm$ 2.07 \\
NGC838 & $\cdots$ & 2.04 $\pm$ 0.20 & 6.39 $\pm$ 0.14 & 16.92 $\pm$ 0.34 & 30.38 $\pm$ 0.61 & 39.34 $\pm$ 0.79 & 48.92 $\pm$ 1.02 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/PhotoTables/Herschel_sigs_stub.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy & \multicolumn{3}{c}{{\sl Herschel}/PACS} & \multicolumn{3}{c}{{\sl Herschel}/SPIRE} \\
ID     & 70\,$\mu$m & 100\,$\mu$m & 160\,$\mu$m & 250\,$\mu$m & 350\,$\mu$m & 500\,$\mu$m \\
       & (Jy) & (Jy) & (Jy) & (Jy) & (Jy) & (Jy) \\
\hline
\multicolumn{7}{c}{Photometry for the SIGS sample} \\
\hline
NGC274 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC275 & 5.96 $\pm$ 0.60 & 8.71 $\pm$ 0.87 & 7.85 $\pm$ 0.79 & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC470 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC474 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC520 & 41.68 $\pm$ 4.17 & 51.86 $\pm$ 5.19 & 39.13 $\pm$ 3.91 & $\cdots$ & $\cdots$ & $\cdots$ \\
IC195 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
IC196 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC833 & 0.39 $\pm$ 0.07 & 0.79 $\pm$ 0.10 & 1.14 $\pm$ 0.12 & 0.58 $\pm$ 0.04 & 0.27 $\pm$ 0.02 & 0.10 $\pm$ 0.01 \\
NGC835 & 7.44 $\pm$ 0.75 & 11.72 $\pm$ 1.17 & 10.58 $\pm$ 1.06 & 4.04 $\pm$ 0.28 & 1.49 $\pm$ 0.10 & 0.46 $\pm$ 0.03 \\
NGC838 & 14.98 $\pm$ 1.50 & 17.84 $\pm$ 1.78 & 12.99 $\pm$ 1.30 & 3.91 $\pm$ 0.27 & 1.37 $\pm$ 0.10 & 0.41 $\pm$ 0.03 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/PhotoTables/WISE_sigs_stub.tex <==
\begin{tabular}{cccccccc}
\hline
Galaxy & \multicolumn{4}{c}{\sl WISE} & \multicolumn{3}{c}{{\sl Spitzer}/MIPS} \\
ID     & 3.4\,$\mu$m & 4.6\,$\mu$m & 12\,$\mu$m & 22\,$\mu$m & 24\,$\mu$m & 70\,$\mu$m & 160\,$\mu$m \\
       & (mJy) & (mJy) & (mJy) & (mJy) & (mJy) & (Jy) & (Jy) \\
\hline
\multicolumn{7}{c}{Photometry for the SIGS sample} \\
\hline
NGC274 & 52.6 $\pm$ 3.2 & 28.3 $\pm$ 1.7 & 11.3 $\pm$ 0.7 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC275 & 38.1 $\pm$ 2.3 & 24.5 $\pm$ 1.5 & 146.5 $\pm$ 8.8 & 384.6 $\pm$ 23.1 & 459.32 $\pm$ 18.39 & 5.40 $\pm$ 0.22 & 7.34 $\pm$ 0.32 \\
NGC470 & 112.5 $\pm$ 6.8 & 69.5 $\pm$ 4.2 & 334.5 $\pm$ 20.1 & 802.2 $\pm$ 48.1 & 799.55 $\pm$ 32.02 & 9.59 $\pm$ 0.39 & 13.72 $\pm$ 0.55 \\
NGC474 & 151.8 $\pm$ 9.1 & 83.3 $\pm$ 5.0 & $\cdots$ & $\cdots$ & 152.39 $\pm$ 8.99 & $\cdots$ & $\cdots$ \\
NGC520 & 183.0 $\pm$ 11.0 & 131.4 $\pm$ 7.9 & 738.3 $\pm$ 44.3 & 2233.4 $\pm$ 134.0 & 2347.72 $\pm$ 93.94 & 33.44 $\pm$ 1.34 & $\cdots$ \\
IC195 & 26.0 $\pm$ 1.6 & 13.9 $\pm$ 0.8 & 4.2 $\pm$ 0.3 & 3.5 $\pm$ 0.3 & $\cdots$ & $\cdots$ & $\cdots$ \\
IC196 & 52.6 $\pm$ 3.2 & 28.4 $\pm$ 1.7 & 37.5 $\pm$ 2.3 & 36.0 $\pm$ 2.2 & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC833 & 51.8 $\pm$ 3.1 & 29.2 $\pm$ 1.7 & 26.7 $\pm$ 1.6 & 49.6 $\pm$ 3.0 & $\cdots$ & $\cdots$ & $\cdots$ \\
NGC835 & 89.9 $\pm$ 5.4 & 56.5 $\pm$ 3.4 & 242.0 $\pm$ 14.5 & 412.1 $\pm$ 24.7 & 434.53 $\pm$ 17.43 & 6.82 $\pm$ 0.27 & 9.33 $\pm$ 0.38 \\
NGC838 & 62.1 $\pm$ 3.7 & 46.2 $\pm$ 2.8 & 459.2 $\pm$ 27.6 & 1344.6 $\pm$ 80.7 & 1458.64 $\pm$ 58.35 & 11.50 $\pm$ 0.46 & 9.60 $\pm$ 0.41 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/4Samples.tex <==
\begin{tabular}{cccl}
\hline
Sample & \# Galaxies& References & Description\\
\hline
SIGS&100& 1,2,3 & Nearby interacting galaxies presented by \citet{2015ApJS..218....6B}.\\
SB&21& 4,5 & Galaxies dominated by star-formation. \\
AGN&29& 5,6,7,8,9,10,11,12,13,14 & Galaxies dominated by AGN.\\
LSM&49$^{\rm a}$& 15,16,17 & Galaxies close to coalescence with a numerical interaction strength of 4 and 5 \citep{2002ApJS..143...47D}. \\
\hline
Total&199$^{\rm b}$&&All galaxies.\\
\hline
\end{tabular}

==> QuantifiyingAGN_arXiv 2/Tables/AGNSample.tex <==
\begin{tabular}{ccrlccr}
\hline
Galaxy & RA & Dec\ \ \  & Redshift & Sample & Size & Angle$^{\rm a}$\\
ID &\multicolumn{2}{c}{(J2000)} & \ \ \ ($z$) & &($\arcsec \times \arcsec$) & ($\degr$)\ \ \ \\
\hline
Mrk 335 & 00:06:19.5 & 20:12:10.5 & 0.0258 & S & 26.9 $\times$ 26.8 & 84.2 \\
Mrk 1502 & 00:53:34.9 & 12:41:36.2 & 0.0589 & S & 29.0 $\times$ 28.5 & 45.0 \\
NGC 931 & 02:28:14.5 & 31:18:42.0 & 0.0167 & S & 100.9 $\times$ 35.7 & 165.7 \\
NGC 1068 & 02:42:40.7 & $-$00:00:47.8 & 0.0038 & HRG & 215.1 $\times$ 174.7 & 170.0 \\
NGC 1194 & 03:03:49.1 & $-$01:06:13.5 & 0.0136 & S & 100.7 $\times$ 42.7 & 50.6 \\
NGC 1320 & 03:24:48.7 & $-$03:02:32.2 & 0.0089 & S & 63.5 $\times$ 33.9 & 47.2 \\
ESO 33$-$2 & 04:55:59.0 & $-$75:32:28.2 & 0.0181 & S & 31.0 $\times$ 29.0 & 45.0 \\
4U 0557$-$385 & 05:58:02.0 & $-$38:20:04.7 & 0.0339 & S & 25.0 $\times$ 23.0 & 229.3 \\
Mrk 3 & 06:15:36.4 & 71:02:15.1 & 0.0135 & S & 48.6 $\times$ 42.9 & 55.0 \\
ESO 428$-$14 & 07:16:31.2 & $-$29:19:29.0 & 0.0057 & S & 46.2 $\times$ 32.0 & 230.0 \\
NGC 3281 & 10:31:52.1 & $-$34:51:13.3 & 0.0107 & S & 114.6 $\times$ 54.7 & 55.0 \\
NGC 3516 & 11:06:47.5 & 72:34:06.9 & 0.0088 & S & 53.3 $\times$ 52.4 & 33.8 \\
NGC 4151 & 12:10:32.6 & 39:24:20.6 & 0.0033 & HR & 256.1 $\times$ 246.5 & 50.0 \\
NGC 4388 & 12:25:46.8 & 12:39:43.5 & 0.0084 & S & 200.7 $\times$ 54.2 & 179.4 \\
Mrk 771 & 12:32:03.6 & 20:09:29.2 & 0.063 & S & 27.8 $\times$ 26.6 & 21.1 \\
NGC 4941 & 13:04:13.1 & $-$05:33:05.8 & 0.0037 & S & 121.6 $\times$ 78.3 & 286.9 \\
MCG $-$03$-$34$-$064 & 13:22:24.5 & $-$16:43:42.5 & 0.0165 & G & 41.5 $\times$ 31.0 & 141.9 \\
ESO 383$-$35 & 13:35:53.7 & $-$34:17:43.9 & 0.0077 & S & 27.9 $\times$ 19.4 & 29.7 \\
ESO 445$-$50 & 13:49:19.3 & $-$30:18:34.0 & 0.0161 & S & 42.0 $\times$ 26.0 & 133.7 \\
NGC 5506 & 14:13:14.9 & $-$03:12:27.3 & 0.0062 & S & 87.3 $\times$ 34.9 & 179.8 \\
2XMM J141348.3$+$440014 & 14:13:48.3 & 44:00:14.0 & 0.0896 & S & 28.0 $\times$ 24.0 & 54.3 \\
NGC 5548 & 14:17:59.5 & 25:08:12.4 & 0.0172 & S & 54.2 $\times$ 44.6 & 190.2 \\
Mrk 1383 & 14:29:06.6 & 01:17:06.5 & 0.0866 & S & 29.2 $\times$ 28.5 & 3.9 \\
Mrk 841 & 15:04:01.2 & 10:26:16.1 & 0.0364 & S & 37.5 $\times$ 34.0 & 105.0 \\
ESO 141$-$55 & 19:21:14.1 & $-$58:40:13.1 & 0.0371 & S & 33.0 $\times$ 29.0 & 0.0 \\
IC 5063 & 20:52:02.3 & $-$57:04:07.6 & 0.0113 & S &79.8 $\times$ 62.6 & 205.1 \\
Mrk 1513 & 21:32:27.8 & 10:08:19.5 & 0.063 & S & 26.2 $\times$ 23.9 & 328.2 \\
Leda 68751 & 22:23:49.5 & $-$02:06:12.8 & 0.0559 & S & 20.0 $\times$ 18.0 & 15.0 \\
NGC 7674 & 23:27:57.0 & 08:46:43.3 & 0.0289 & HRG & 50.0 $\times$ 50.0 & 0.0 \\
\hline
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPAr1_SIGS_stub.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
NGC275 & 0.20 $\pm$ 0.14 & $9.26 \pm 0.30$ & $9.42 \pm 0.09$ & $9.57 \pm 0.07$ & 2.09 $\pm$ 0.18 & $9.84 \pm 0.07$ \\
NGC470 & $\cdots$ & $\cdots$ & $10.22 \pm 0.02$ & $10.04 \pm 0.03$ & 2.00 $\pm$ 0.10 & $10.47 \pm 0.02$ \\
NGC474 & $\cdots$ & $\cdots$ & $9.65 \pm 0.05$ & $8.94 \pm 0.06$ & 2.04 $\pm$ 0.10 & $9.74 \pm 0.04$ \\
NGC520 & 0.58 $\pm$ 0.08 & $10.69 \pm 0.07$ & $10.45 \pm 0.06$ & $9.81 \pm 0.16$ & 2.37 $\pm$ 0.28 & $10.56 \pm 0.08$ \\
IC196 & $\cdots$ & $\cdots$ & $9.66 \pm 0.02$ & $8.82 \pm 0.02$ & 2.32 $\pm$ 0.12 & $9.73 \pm 0.02$ \\
NGC833 & 0.27 $\pm$ 0.07 & $9.09 \pm 0.15$ & $9.50 \pm 0.02$ & $8.11 \pm 0.17$ & 2.87 $\pm$ 0.17 & $9.52 \pm 0.02$ \\
NGC835 & $\cdots$ & $\cdots$ & $10.60 \pm 0.04$ & $10.12 \pm 0.07$ & 2.00 $\pm$ 0.10 & $10.74 \pm 0.02$ \\
NGC838 & $\cdots$ & $\cdots$ & $10.71 \pm 0.02$ & $10.48 \pm 0.04$ & 1.75 $\pm$ 0.09 & $10.94 \pm 0.02$ \\
NGC839 & $\cdots$ & $\cdots$ & $10.70 \pm 0.02$ & $10.48 \pm 0.03$ & 1.50 $\pm$ 0.07 & $10.93 \pm 0.02$ \\
NGC935 & $\cdots$ & $\cdots$ & $10.54 \pm 0.02$ & $10.11 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.70 \pm 0.02$ \\
IC1801 & $\cdots$ & $\cdots$ & $10.06 \pm 0.02$ & $9.77 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.27 \pm 0.02$ \\
NGC1241 & 0.21 $\pm$ 0.09 & $10.13 \pm 0.18$ & $10.57 \pm 0.05$ & $10.09 \pm 0.07$ & 2.54 $\pm$ 0.27 & $10.71 \pm 0.05$ \\
NGC1242 & 0.41 $\pm$ 0.08 & $9.44 \pm 0.09$ & $9.40 \pm 0.07$ & $9.09 \pm 0.14$ & 2.68 $\pm$ 0.23 & $9.60 \pm 0.05$ \\
NGC1253 & 0.21 $\pm$ 0.09 & $9.20 \pm 0.18$ & $9.61 \pm 0.14$ & $9.19 \pm 0.22$ & 2.57 $\pm$ 0.27 & $9.77 \pm 0.05$ \\
NGC1253A & $\cdots$ & $\cdots$ & $8.22 \pm 0.03$ & $8.58 \pm 0.02$ & 1.75 $\pm$ 0.09 & $8.79 \pm 0.02$ \\
NGC2276 & 0.20 $\pm$ 0.08 & $10.13 \pm 0.18$ & $10.40 \pm 0.06$ & $10.38 \pm 0.06$ & 2.44 $\pm$ 0.24 & $10.73 \pm 0.04$ \\
NGC2444 & $\cdots$ & $\cdots$ & $9.05 \pm 0.02$ & $8.00 \pm 0.09$ & 2.00 $\pm$ 0.10 & $9.10 \pm 0.02$ \\
NGC2445 & $\cdots$ & $\cdots$ & $10.28 \pm 0.05$ & $10.24 \pm 0.05$ & 1.97 $\pm$ 0.10 & $10.59 \pm 0.02$ \\
NGC2633 & $\cdots$ & $\cdots$ & $10.40 \pm 0.02$ & $10.32 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.70 \pm 0.02$ \\
NGC2634 & $\cdots$ & $\cdots$ & $8.64 \pm 0.02$ & $7.04 \pm 0.36$ & 2.96 $\pm$ 0.15 & $8.65 \pm 0.02$ \\
NGC2719A & $\cdots$ & $\cdots$ & $8.65 \pm 0.06$ & $9.19 \pm 0.02$ & 1.50 $\pm$ 0.07 & $9.35 \pm 0.02$ \\
NGC2719 & 0.26 $\pm$ 0.11 & $8.88 \pm 0.22$ & $8.80 \pm 0.14$ & $9.10 \pm 0.05$ & 1.88 $\pm$ 0.13 & $9.32 \pm 0.07$ \\
NGC2805 & $\cdots$ & $\cdots$ & $9.38 \pm 0.04$ & $9.51 \pm 0.02$ & 2.47 $\pm$ 0.12 & $9.79 \pm 0.02$ \\
NGC2814 & 0.42 $\pm$ 0.11 & $8.86 \pm 0.12$ & $8.69 \pm 0.08$ & $8.63 \pm 0.13$ & 2.54 $\pm$ 0.30 & $8.99 \pm 0.08$ \\
NGC2820A & $\cdots$ & $\cdots$ & $7.69 \pm 0.02$ & $8.21 \pm 0.02$ & 1.69 $\pm$ 0.11 & $8.37 \pm 0.02$ \\
NGC2820 & 0.25 $\pm$ 0.07 & $9.24 \pm 0.13$ & $9.46 \pm 0.04$ & $9.29 \pm 0.05$ & 2.47 $\pm$ 0.20 & $9.72 \pm 0.04$ \\
NGC2964 & 0.22 $\pm$ 0.08 & $9.57 \pm 0.16$ & $9.82 \pm 0.06$ & $9.71 \pm 0.03$ & 2.23 $\pm$ 0.16 & $10.10 \pm 0.04$ \\
NGC2970 & $\cdots$ & $\cdots$ & $7.89 \pm 0.02$ & $6.86 \pm 0.02$ & 1.17 $\pm$ 0.18 & $7.94 \pm 0.02$ \\
NGC2976 & 0.29 $\pm$ 0.04 & $8.32 \pm 0.06$ & $8.42 \pm 0.05$ & $8.31 \pm 0.05$ & 2.91 $\pm$ 0.15 & $8.70 \pm 0.03$ \\
NGC3031 & $\cdots$ & $\cdots$ & $9.46 \pm 0.02$ & $8.76 \pm 0.02$ & 2.96 $\pm$ 0.15 & $9.55 \pm 0.02$ \\
NGC3034 & 0.48 $\pm$ 0.03 & $10.19 \pm 0.05$ & $10.20 \pm 0.02$ & $8.46 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.21 \pm 0.02$ \\
NGC3077 & 0.30 $\pm$ 0.07 & $8.30 \pm 0.11$ & $8.45 \pm 0.09$ & $8.18 \pm 0.11$ & 2.00 $\pm$ 0.10 & $8.66 \pm 0.03$ \\
NGC3165 & $\cdots$ & $\cdots$ & $7.86 \pm 0.09$ & $8.04 \pm 0.05$ & 2.01 $\pm$ 0.10 & $8.30 \pm 0.02$ \\
NGC3166 & 0.21 $\pm$ 0.04 & $9.06 \pm 0.09$ & $9.60 \pm 0.02$ & $8.36 \pm 0.02$ & 2.56 $\pm$ 0.14 & $9.63 \pm 0.02$ \\
NGC3169 & $\cdots$ & $\cdots$ & $10.04 \pm 0.06$ & $9.38 \pm 0.27$ & 2.71 $\pm$ 0.19 & $10.14 \pm 0.03$ \\
NGC3185 & $\cdots$ & $\cdots$ & $9.12 \pm 0.02$ & $8.81 \pm 0.02$ & 2.25 $\pm$ 0.11 & $9.32 \pm 0.02$ \\
NGC3187 & 0.21 $\pm$ 0.05 & $8.64 \pm 0.11$ & $8.91 \pm 0.04$ & $8.86 \pm 0.02$ & 2.95 $\pm$ 0.15 & $9.22 \pm 0.02$ \\
NGC3190 & $\cdots$ & $\cdots$ & $9.73 \pm 0.02$ & $8.22 \pm 0.03$ & 2.50 $\pm$ 0.13 & $9.74 \pm 0.02$ \\
NGC3226 & $\cdots$ & $\cdots$ & $8.79 \pm 0.02$ & $7.49 \pm 0.24$ & 2.26 $\pm$ 0.11 & $8.82 \pm 0.02$ \\
NGC3227 & 0.20 $\pm$ 0.03 & $9.32 \pm 0.08$ & $9.76 \pm 0.04$ & $9.30 \pm 0.03$ & 2.26 $\pm$ 0.11 & $9.91 \pm 0.02$ \\
NGC3395 & $\cdots$ & $\cdots$ & $9.52 \pm 0.08$ & $9.65 \pm 0.07$ & 2.00 $\pm$ 0.10 & $9.93 \pm 0.02$ \\
NGC3396 & $\cdots$ & $\cdots$ & $9.52 \pm 0.04$ & $9.70 \pm 0.02$ & 1.75 $\pm$ 0.09 & $9.96 \pm 0.02$ \\
NGC3424 & $\cdots$ & $\cdots$ & $9.89 \pm 0.02$ & $9.62 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.10 \pm 0.02$ \\
NGC3430 & $\cdots$ & $\cdots$ & $9.61 \pm 0.03$ & $9.67 \pm 0.02$ & 2.39 $\pm$ 0.12 & $9.98 \pm 0.02$ \\
NGC3448 & 0.40 $\pm$ 0.05 & $9.46 \pm 0.07$ & $9.20 \pm 0.05$ & $9.36 \pm 0.04$ & 2.27 $\pm$ 0.11 & $9.63 \pm 0.03$ \\
IC694 & $\cdots$ & $\cdots$ & $9.02 \pm 0.06$ & $7.54 \pm 0.03$ & 1.24 $\pm$ 0.19 & $9.03 \pm 0.06$ \\
NGC3690 & $\cdots$ & $\cdots$ & $11.47 \pm 0.02$ & $11.51 \pm 0.03$ & 1.25 $\pm$ 0.06 & $11.83 \pm 0.02$ \\
NGC3786 & 0.22 $\pm$ 0.08 & $9.39 \pm 0.16$ & $9.75 \pm 0.05$ & $9.36 \pm 0.03$ & 2.22 $\pm$ 0.11 & $9.92 \pm 0.04$ \\
NGC3788 & $\cdots$ & $\cdots$ & $9.86 \pm 0.02$ & $9.45 \pm 0.07$ & 2.29 $\pm$ 0.11 & $10.02 \pm 0.02$ \\
NGC3799 & $\cdots$ & $\cdots$ & $9.27 \pm 0.08$ & $9.26 \pm 0.08$ & 2.25 $\pm$ 0.11 & $9.60 \pm 0.02$ \\
NGC3800 & $\cdots$ & $\cdots$ & $10.36 \pm 0.03$ & $10.09 \pm 0.02$ & 2.23 $\pm$ 0.11 & $10.57 \pm 0.02$ \\
IC749 & $\cdots$ & $\cdots$ & $8.61 \pm 0.05$ & $8.74 \pm 0.04$ & 2.25 $\pm$ 0.11 & $9.02 \pm 0.02$ \\
IC750 & 0.33 $\pm$ 0.07 & $9.32 \pm 0.11$ & $9.52 \pm 0.04$ & $8.88 \pm 0.04$ & 2.65 $\pm$ 0.26 & $9.62 \pm 0.04$ \\
NGC4038 & $\cdots$ & $\cdots$ & $10.61 \pm 0.04$ & $10.55 \pm 0.04$ & 2.00 $\pm$ 0.10 & $10.91 \pm 0.02$ \\
NGC4394 & $\cdots$ & $\cdots$ & $9.08 \pm 0.03$ & $8.26 \pm 0.02$ & 2.59 $\pm$ 0.21 & $9.15 \pm 0.02$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPAr2_PsiAGN.tex <==
\begin{tabular}{cccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
Mrk335 & $-0.94 \pm 0.91$ & $8.51 \pm 0.53$ & $9.58 \pm 0.14$ & $10.08 \pm 0.17$ & $10.47 \pm 0.16$ \\
Mrk771 & $0.51 \pm 0.24$ & $8.94 \pm 0.22$ & $9.47 \pm 0.12$ & $10.47 \pm 0.16$ & $10.88 \pm 0.14$ \\
2XMMJ141348.3+440014 & $0.56 \pm 0.40$ & $9.31 \pm 0.52$ & $9.34 \pm 0.30$ & $10.27 \pm 0.45$ & $10.68 \pm 0.41$ \\
Mrk1383 & $1.31 \pm 0.21$ & $9.00 \pm 0.39$ & $9.24 \pm 0.22$ & $10.68 \pm 0.19$ & $11.14 \pm 0.15$ \\
ESO141-55 & $0.12 \pm 0.68$ & $8.60 \pm 0.47$ & $9.49 \pm 0.21$ & $10.66 \pm 0.22$ & $11.06 \pm 0.19$ \\
Mrk1513 & $0.18 \pm 0.65$ & $8.72 \pm 0.67$ & $9.51 \pm 0.19$ & $10.68 \pm 0.24$ & $11.08 \pm 0.22$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar1_AGN.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
Mrk335 & 0.77 $\pm$ 0.04 & $11.03 \pm 0.02$ & $9.42 \pm 0.15$ & $9.78 \pm 0.07$ & 1.03 $\pm$ 0.08 & $9.99 \pm 0.05$ \\
Mrk1502 & 0.49 $\pm$ 0.03 & $11.72 \pm 0.02$ & $11.28 \pm 0.05$ & $11.31 \pm 0.04$ & 1.52 $\pm$ 0.08 & $11.64 \pm 0.03$ \\
NGC931 & 0.51 $\pm$ 0.04 & $10.68 \pm 0.04$ & $10.50 \pm 0.04$ & $9.95 \pm 0.07$ & 2.68 $\pm$ 0.21 & $10.62 \pm 0.04$ \\
NGC1068 & 0.42 $\pm$ 0.07 & $10.93 \pm 0.08$ & $10.86 \pm 0.07$ & $10.56 \pm 0.11$ & 2.01 $\pm$ 0.10 & $11.06 \pm 0.05$ \\
NGC1194 & 0.66 $\pm$ 0.07 & $10.17 \pm 0.05$ & $9.83 \pm 0.08$ & $8.06 \pm 0.44$ & 2.20 $\pm$ 0.24 & $9.84 \pm 0.08$ \\
NGC1320 & 0.43 $\pm$ 0.06 & $9.85 \pm 0.05$ & $9.87 \pm 0.06$ & $9.08 \pm 0.30$ & 1.89 $\pm$ 0.12 & $9.95 \pm 0.07$ \\
ESO33-2 & 0.63 $\pm$ 0.03 & $10.33 \pm 0.02$ & $10.02 \pm 0.03$ & $7.99 \pm 0.59$ & 1.75 $\pm$ 0.09 & $10.03 \pm 0.03$ \\
4U0557-385 & 0.90 $\pm$ 0.04 & $11.25 \pm 0.02$ & $10.14 \pm 0.04$ & $9.32 \pm 0.19$ & 1.84 $\pm$ 0.12 & $10.21 \pm 0.02$ \\
Mrk3 & 0.64 $\pm$ 0.06 & $10.62 \pm 0.03$ & $10.34 \pm 0.08$ & $8.75 \pm 0.04$ & 1.63 $\pm$ 0.13 & $10.36 \pm 0.08$ \\
ESO428-14 & 0.31 $\pm$ 0.04 & $9.50 \pm 0.06$ & $9.77 \pm 0.07$ & $8.89 \pm 0.44$ & 1.74 $\pm$ 0.09 & $9.83 \pm 0.03$ \\
NGC3281 & 0.40 $\pm$ 0.05 & $10.37 \pm 0.07$ & $10.52 \pm 0.03$ & $8.25 \pm 0.99$ & 1.75 $\pm$ 0.09 & $10.52 \pm 0.03$ \\
NGC3516 & 0.45 $\pm$ 0.03 & $10.12 \pm 0.05$ & $9.85 \pm 0.04$ & $7.98 \pm 1.06$ & 1.44 $\pm$ 0.11 & $9.86 \pm 0.03$ \\
NGC4151 & 0.67 $\pm$ 0.07 & $9.86 \pm 0.08$ & $9.25 \pm 0.19$ & $8.92 \pm 0.20$ & 2.18 $\pm$ 0.19 & $9.44 \pm 0.07$ \\
NGC4388 & 0.24 $\pm$ 0.04 & $10.14 \pm 0.08$ & $10.49 \pm 0.03$ & $10.00 \pm 0.05$ & 2.01 $\pm$ 0.10 & $10.63 \pm 0.02$ \\
Mrk771 & 0.53 $\pm$ 0.03 & $11.47 \pm 0.04$ & $10.63 \pm 0.07$ & $9.06 \pm 1.66$ & 1.68 $\pm$ 0.11 & $10.64 \pm 0.04$ \\
NGC4941 & $\cdots$ & $\cdots$ & $9.39 \pm 0.02$ & $8.40 \pm 0.02$ & 2.71 $\pm$ 0.20 & $9.44 \pm 0.02$ \\
MCG-03-34-064 & 0.46 $\pm$ 0.04 & $10.69 \pm 0.06$ & $10.67 \pm 0.05$ & $9.82 \pm 0.29$ & 1.49 $\pm$ 0.07 & $10.74 \pm 0.03$ \\
ESO383-35 & 0.65 $\pm$ 0.04 & $9.85 \pm 0.03$ & $9.47 \pm 0.05$ & $8.31 \pm 0.30$ & 1.33 $\pm$ 0.12 & $9.51 \pm 0.06$ \\
ESO445-50 & 0.81 $\pm$ 0.04 & $10.99 \pm 0.02$ & $10.28 \pm 0.05$ & $8.18 \pm 0.56$ & 1.55 $\pm$ 0.10 & $10.29 \pm 0.05$ \\
NGC5506 & 0.56 $\pm$ 0.03 & $10.25 \pm 0.03$ & $10.05 \pm 0.02$ & $8.94 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.09 \pm 0.02$ \\
2XMMJ141348.3+440014 & 0.85 $\pm$ 0.04 & $11.89 \pm 0.13$ & $10.09 \pm 0.27$ & $10.36 \pm 0.16$ & 2.02 $\pm$ 0.10 & $10.59 \pm 0.04$ \\
NGC5548 & 0.54 $\pm$ 0.08 & $10.46 \pm 0.09$ & $10.13 \pm 0.15$ & $9.47 \pm 0.33$ & 1.92 $\pm$ 0.15 & $10.23 \pm 0.07$ \\
Mrk1383 & 0.65 $\pm$ 0.03 & $12.11 \pm 0.02$ & $11.04 \pm 0.03$ & $9.33 \pm 1.13$ & 1.75 $\pm$ 0.09 & $11.05 \pm 0.02$ \\
Mrk841 & 0.64 $\pm$ 0.03 & $11.08 \pm 0.02$ & $9.78 \pm 0.03$ & $10.31 \pm 0.02$ & 1.00 $\pm$ 0.05 & $10.48 \pm 0.02$ \\
ESO141-55 & 0.52 $\pm$ 0.03 & $11.33 \pm 0.10$ & $10.20 \pm 0.25$ & $10.57 \pm 0.09$ & 2.00 $\pm$ 0.10 & $10.77 \pm 0.02$ \\
IC5063 & 0.70 $\pm$ 0.03 & $10.67 \pm 0.02$ & $10.28 \pm 0.02$ & $8.59 \pm 0.26$ & 2.00 $\pm$ 0.10 & $10.29 \pm 0.02$ \\
Mrk1513 & 0.66 $\pm$ 0.03 & $11.69 \pm 0.04$ & $10.48 \pm 0.11$ & $10.78 \pm 0.05$ & 1.52 $\pm$ 0.08 & $11.00 \pm 0.02$ \\
LEDA68751 & 0.80 $\pm$ 0.04 & $11.35 \pm 0.03$ & $10.32 \pm 0.14$ & $10.13 \pm 0.19$ & 1.21 $\pm$ 0.15 & $10.57 \pm 0.04$ \\
NGC7674 & 0.27 $\pm$ 0.05 & $11.03 \pm 0.08$ & $11.23 \pm 0.05$ & $10.92 \pm 0.04$ & 1.77 $\pm$ 0.09 & $11.43 \pm 0.04$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar1_LSM.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
NGC0078 & $\cdots$ & $\cdots$ & $10.03 \pm 0.02$ & $9.27 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.11 \pm 0.02$ \\
UM246 & 0.25 $\pm$ 0.09 & $10.36 \pm 0.16$ & $10.48 \pm 0.09$ & $10.49 \pm 0.07$ & 2.20 $\pm$ 0.22 & $10.82 \pm 0.07$ \\
2MASXJ01221811+0100262 & 0.42 $\pm$ 0.10 & $11.27 \pm 0.12$ & $11.06 \pm 0.06$ & $11.05 \pm 0.07$ & 1.75 $\pm$ 0.09 & $11.40 \pm 0.06$ \\
CGCG087-046 & 0.51 $\pm$ 0.06 & $11.07 \pm 0.06$ & $10.86 \pm 0.06$ & $10.54 \pm 0.08$ & 2.78 $\pm$ 0.20 & $11.06 \pm 0.04$ \\
UGC04383 & 0.22 $\pm$ 0.04 & $9.89 \pm 0.11$ & $10.09 \pm 0.05$ & $10.11 \pm 0.04$ & 2.00 $\pm$ 0.10 & $10.44 \pm 0.02$ \\
2MASXJ08343370+1720462 & 0.52 $\pm$ 0.06 & $10.55 \pm 0.06$ & $10.34 \pm 0.06$ & $9.95 \pm 0.09$ & 2.29 $\pm$ 0.12 & $10.51 \pm 0.05$ \\
2MASXJ08381760+3054533 & 0.22 $\pm$ 0.10 & $10.03 \pm 0.20$ & $10.51 \pm 0.04$ & $9.64 \pm 0.27$ & 2.12 $\pm$ 0.13 & $10.57 \pm 0.05$ \\
2MASXJ08434495+3549421 & 0.49 $\pm$ 0.10 & $10.53 \pm 0.10$ & $10.34 \pm 0.10$ & $9.98 \pm 0.05$ & 1.87 $\pm$ 0.15 & $10.52 \pm 0.08$ \\
UGC05044 & 0.50 $\pm$ 0.09 & $10.59 \pm 0.08$ & $10.40 \pm 0.09$ & $10.05 \pm 0.06$ & 2.50 $\pm$ 0.32 & $10.59 \pm 0.08$ \\
ARP142 & 0.29 $\pm$ 0.05 & $10.41 \pm 0.08$ & $10.65 \pm 0.04$ & $10.22 \pm 0.02$ & 2.82 $\pm$ 0.19 & $10.80 \pm 0.03$ \\
CGCG266-026 & $\cdots$ & $\cdots$ & $10.81 \pm 0.04$ & $10.44 \pm 0.08$ & 2.37 $\pm$ 0.13 & $10.99 \pm 0.02$ \\
LSBCF567-01 & $\cdots$ & $\cdots$ & $7.63 \pm 0.02$ & $8.13 \pm 0.02$ & 1.75 $\pm$ 0.09 & $8.30 \pm 0.02$ \\
2MASXJ10225654+3446467 & 0.54 $\pm$ 0.12 & $10.51 \pm 0.11$ & $10.36 \pm 0.11$ & $9.53 \pm 0.16$ & 2.48 $\pm$ 0.31 & $10.43 \pm 0.11$ \\
UGC05644 & $\cdots$ & $\cdots$ & $10.57 \pm 0.04$ & $10.21 \pm 0.02$ & 2.23 $\pm$ 0.11 & $10.75 \pm 0.02$ \\
CGCG037-076 & $\cdots$ & $\cdots$ & $10.44 \pm 0.05$ & $10.68 \pm 0.04$ & 1.26 $\pm$ 0.08 & $10.93 \pm 0.03$ \\
UGCA219 & $\cdots$ & $\cdots$ & $8.19 \pm 0.02$ & $8.70 \pm 0.02$ & 1.26 $\pm$ 0.06 & $8.87 \pm 0.02$ \\
NGC3445 & 0.24 $\pm$ 0.05 & $9.12 \pm 0.10$ & $8.94 \pm 0.03$ & $9.46 \pm 0.02$ & 2.24 $\pm$ 0.11 & $9.62 \pm 0.02$ \\
2MASXJ10591815+2432343 & 0.24 $\pm$ 0.04 & $11.27 \pm 0.09$ & $11.47 \pm 0.02$ & $11.40 \pm 0.02$ & 1.75 $\pm$ 0.09 & $11.78 \pm 0.02$ \\
VV627 & $\cdots$ & $\cdots$ & $10.63 \pm 0.04$ & $10.28 \pm 0.02$ & 2.25 $\pm$ 0.11 & $10.82 \pm 0.02$ \\
IC0700 & $\cdots$ & $\cdots$ & $7.98 \pm 0.02$ & $8.41 \pm 0.02$ & 1.75 $\pm$ 0.09 & $8.60 \pm 0.02$ \\
UGC06665 & $\cdots$ & $\cdots$ & $10.45 \pm 0.04$ & $10.60 \pm 0.03$ & 1.50 $\pm$ 0.07 & $10.88 \pm 0.02$ \\
UGC07388 & 0.21 $\pm$ 0.08 & $9.78 \pm 0.18$ & $10.23 \pm 0.05$ & $9.68 \pm 0.08$ & 2.37 $\pm$ 0.17 & $10.35 \pm 0.04$ \\
NGC4320 & 0.46 $\pm$ 0.14 & $10.20 \pm 0.13$ & $10.03 \pm 0.13$ & $9.80 \pm 0.10$ & 2.73 $\pm$ 0.34 & $10.26 \pm 0.11$ \\
UGC07936 & 0.38 $\pm$ 0.08 & $9.94 \pm 0.10$ & $9.74 \pm 0.11$ & $9.87 \pm 0.06$ & 2.75 $\pm$ 0.26 & $10.15 \pm 0.06$ \\
MRK0237 & 0.30 $\pm$ 0.06 & $10.38 \pm 0.10$ & $10.31 \pm 0.04$ & $10.47 \pm 0.04$ & 2.00 $\pm$ 0.10 & $10.74 \pm 0.03$ \\
UGC08327 & 0.28 $\pm$ 0.07 & $10.67 \pm 0.10$ & $10.81 \pm 0.05$ & $10.59 \pm 0.11$ & 1.77 $\pm$ 0.09 & $11.04 \pm 0.04$ \\
UGC08335 & $\cdots$ & $\cdots$ & $11.38 \pm 0.05$ & $11.41 \pm 0.07$ & 1.40 $\pm$ 0.12 & $11.74 \pm 0.06$ \\
NGC5100 & 0.28 $\pm$ 0.07 & $10.63 \pm 0.11$ & $10.89 \pm 0.05$ & $10.40 \pm 0.08$ & 2.30 $\pm$ 0.12 & $11.03 \pm 0.04$ \\
CGCG017-018 & $\cdots$ & $\cdots$ & $10.60 \pm 0.02$ & $10.52 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.89 \pm 0.02$ \\
NGC5331 & 0.24 $\pm$ 0.13 & $10.97 \pm 0.24$ & $11.25 \pm 0.08$ & $10.97 \pm 0.09$ & 2.13 $\pm$ 0.13 & $11.46 \pm 0.08$ \\
UGC09618 & $\cdots$ & $\cdots$ & $11.42 \pm 0.09$ & $10.95 \pm 0.26$ & 2.25 $\pm$ 0.11 & $11.57 \pm 0.02$ \\
2MASXJ15015015+2332536 & 0.33 $\pm$ 0.08 & $10.41 \pm 0.12$ & $10.54 \pm 0.05$ & $10.16 \pm 0.11$ & 2.30 $\pm$ 0.15 & $10.72 \pm 0.05$ \\
SBS1509+583 & $\cdots$ & $\cdots$ & $10.22 \pm 0.04$ & $9.77 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.37 \pm 0.02$ \\
KUG1553+200 & $\cdots$ & $\cdots$ & $10.76 \pm 0.03$ & $10.70 \pm 0.03$ & 1.75 $\pm$ 0.09 & $11.07 \pm 0.02$ \\
KUG1556+326 & 0.26 $\pm$ 0.11 & $10.23 \pm 0.21$ & $10.49 \pm 0.06$ & $10.14 \pm 0.09$ & 2.28 $\pm$ 0.13 & $10.67 \pm 0.05$ \\
MRK0881 & 0.32 $\pm$ 0.06 & $10.35 \pm 0.09$ & $10.23 \pm 0.05$ & $10.40 \pm 0.03$ & 2.00 $\pm$ 0.10 & $10.67 \pm 0.03$ \\
2MASXJ17045097+3449020 & $\cdots$ & $\cdots$ & $11.19 \pm 0.02$ & $11.07 \pm 0.02$ & 1.75 $\pm$ 0.09 & $11.47 \pm 0.02$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar1_PsiAGN.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
Mrk335 & 0.86 $\pm$ 0.04 & $11.14 \pm 0.02$ & $9.88 \pm 0.07$ & $8.53 \pm 0.90$ & 1.06 $\pm$ 0.16 & $9.90 \pm 0.06$ \\
Mrk771 & 0.81 $\pm$ 0.04 & $11.43 \pm 0.02$ & $10.18 \pm 0.13$ & $9.84 \pm 0.23$ & 2.24 $\pm$ 0.29 & $10.37 \pm 0.09$ \\
2XMMJ141348.3+440014 & 0.90 $\pm$ 0.04 & $11.96 \pm 0.02$ & $10.30 \pm 0.18$ & $9.95 \pm 0.35$ & 2.33 $\pm$ 0.25 & $10.49 \pm 0.04$ \\
Mrk1383 & 0.80 $\pm$ 0.04 & $12.00 \pm 0.04$ & $10.52 \pm 0.25$ & $10.59 \pm 0.20$ & 2.05 $\pm$ 0.16 & $10.89 \pm 0.05$ \\
ESO141-55 & 0.74 $\pm$ 0.04 & $11.56 \pm 0.02$ & $10.52 \pm 0.10$ & $9.55 \pm 0.64$ & 2.56 $\pm$ 0.21 & $10.57 \pm 0.06$ \\
Mrk1513 & 0.86 $\pm$ 0.04 & $11.87 \pm 0.02$ & $10.61 \pm 0.11$ & $9.65 \pm 0.63$ & 2.13 $\pm$ 0.23 & $10.66 \pm 0.07$ \\
\hline
\end{tabular}

==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar1_SB.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
NGC23 & 0.32 $\pm$ 0.06 & $10.60 \pm 0.10$ & $10.73 \pm 0.04$ & $10.39 \pm 0.06$ & 2.02 $\pm$ 0.10 & $10.92 \pm 0.04$ \\
NGC253 & 0.23 $\pm$ 0.12 & $9.96 \pm 0.22$ & $10.32 \pm 0.04$ & $9.95 \pm 0.15$ & 2.38 $\pm$ 0.21 & $10.50 \pm 0.07$ \\
NGC660 & 0.43 $\pm$ 0.08 & $10.14 \pm 0.09$ & $10.14 \pm 0.04$ & $9.59 \pm 0.13$ & 2.32 $\pm$ 0.25 & $10.26 \pm 0.05$ \\
NGC1222 & $\cdots$ & $\cdots$ & $10.35 \pm 0.02$ & $10.31 \pm 0.02$ & 1.50 $\pm$ 0.07 & $10.66 \pm 0.02$ \\
NGC1365 & 0.39 $\pm$ 0.12 & $10.87 \pm 0.14$ & $10.83 \pm 0.10$ & $10.60 \pm 0.16$ & 2.58 $\pm$ 0.34 & $11.06 \pm 0.08$ \\
IC342 & $\cdots$ & $\cdots$ & $8.39 \pm 0.03$ & $7.49 \pm 0.24$ & 2.26 $\pm$ 0.11 & $8.45 \pm 0.02$ \\
NGC1614 & $\cdots$ & $\cdots$ & $11.31 \pm 0.04$ & $11.24 \pm 0.05$ & 1.37 $\pm$ 0.12 & $11.61 \pm 0.04$ \\
NGC1797 & $\cdots$ & $\cdots$ & $10.63 \pm 0.07$ & $10.68 \pm 0.05$ & 1.75 $\pm$ 0.09 & $11.00 \pm 0.02$ \\
NGC2146 & 0.38 $\pm$ 0.04 & $10.41 \pm 0.06$ & $10.60 \pm 0.04$ & $9.09 \pm 0.77$ & 2.00 $\pm$ 0.10 & $10.62 \pm 0.02$ \\
NGC2623 & 0.27 $\pm$ 0.06 & $10.72 \pm 0.11$ & $10.83 \pm 0.04$ & $10.78 \pm 0.05$ & 1.73 $\pm$ 0.09 & $11.14 \pm 0.04$ \\
NGC3256 & $\cdots$ & $\cdots$ & $11.30 \pm 0.02$ & $11.21 \pm 0.02$ & 1.75 $\pm$ 0.09 & $11.59 \pm 0.02$ \\
NGC3310 & 0.20 $\pm$ 0.07 & $9.61 \pm 0.16$ & $9.63 \pm 0.05$ & $10.00 \pm 0.04$ & 1.94 $\pm$ 0.11 & $10.20 \pm 0.03$ \\
NGC3556 & 0.28 $\pm$ 0.09 & $9.53 \pm 0.15$ & $9.71 \pm 0.05$ & $9.47 \pm 0.09$ & 2.65 $\pm$ 0.29 & $9.93 \pm 0.06$ \\
NGC3628 & 0.22 $\pm$ 0.03 & $9.85 \pm 0.07$ & $10.34 \pm 0.02$ & $9.29 \pm 0.06$ & 2.93 $\pm$ 0.15 & $10.39 \pm 0.02$ \\
NGC4088 & $\cdots$ & $\cdots$ & $9.85 \pm 0.03$ & $9.64 \pm 0.02$ & 2.01 $\pm$ 0.10 & $10.09 \pm 0.02$ \\
NGC4194 & $\cdots$ & $\cdots$ & $10.59 \pm 0.02$ & $10.50 \pm 0.02$ & 1.50 $\pm$ 0.07 & $10.88 \pm 0.02$ \\
Mrk52 & $\cdots$ & $\cdots$ & $9.87 \pm 0.04$ & $9.91 \pm 0.03$ & 1.75 $\pm$ 0.09 & $10.23 \pm 0.03$ \\
NGC4676 & $\cdots$ & $\cdots$ & $10.72 \pm 0.02$ & $10.36 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.90 \pm 0.02$ \\
NGC4818 & 0.24 $\pm$ 0.09 & $9.53 \pm 0.19$ & $9.89 \pm 0.05$ & $9.33 \pm 0.09$ & 1.82 $\pm$ 0.15 & $10.02 \pm 0.05$ \\
NGC4945 & $\cdots$ & $\cdots$ & $10.77 \pm 0.17$ & $10.60 \pm 0.21$ & 2.27 $\pm$ 0.11 & $11.02 \pm 0.02$ \\
NGC7252 & $\cdots$ & $\cdots$ & $10.60 \pm 0.03$ & $10.23 \pm 0.04$ & 2.00 $\pm$ 0.10 & $10.78 \pm 0.02$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar2_AGN.tex <==
\begin{tabular}{cccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
Mrk335 & $0.49 \pm 0.09$ & $9.60 \pm 0.28$ & $8.34 \pm 0.44$ & $8.29 \pm 0.64$ & $8.94 \pm 0.37$ \\
Mrk1502 & $1.86 \pm 0.03$ & $9.56 \pm 0.33$ & $8.92 \pm 0.20$ & $10.40 \pm 0.17$ & $10.93 \pm 0.13$ \\
NGC931 & $0.49 \pm 0.05$ & $8.99 \pm 0.04$ & $9.61 \pm 0.02$ & $10.77 \pm 0.02$ & $11.16 \pm 0.02$ \\
NGC1068 & $1.07 \pm 0.11$ & $8.95 \pm 0.10$ & $9.36 \pm 0.07$ & $10.70 \pm 0.09$ & $11.13 \pm 0.08$ \\
NGC1194 & $-1.31 \pm 0.42$ & $8.47 \pm 0.33$ & $9.55 \pm 0.09$ & $10.45 \pm 0.07$ & $10.84 \pm 0.06$ \\
NGC1320 & $-0.37 \pm 0.25$ & $8.81 \pm 0.15$ & $9.52 \pm 0.06$ & $10.15 \pm 0.03$ & $10.56 \pm 0.02$ \\
ESO33-2 & $-1.46 \pm 0.58$ & $8.39 \pm 0.40$ & $9.56 \pm 0.12$ & $10.48 \pm 0.10$ & $10.88 \pm 0.09$ \\
4U0557-385 & $-0.06 \pm 0.11$ & $8.72 \pm 0.12$ & $9.48 \pm 0.04$ & $10.61 \pm 0.07$ & $11.02 \pm 0.07$ \\
Mrk3 & $-0.74 \pm 0.03$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.77 \pm 0.02$ & $11.16 \pm 0.02$ \\
ESO428-14 & $-0.59 \pm 0.43$ & $8.72 \pm 0.39$ & $9.40 \pm 0.27$ & $9.85 \pm 0.18$ & $10.28 \pm 0.13$ \\
NGC3281 & $-1.19 \pm 0.93$ & $8.21 \pm 0.52$ & $9.40 \pm 0.16$ & $10.71 \pm 0.11$ & $11.12 \pm 0.09$ \\
NGC3516 & $-1.35 \pm 1.11$ & $8.26 \pm 0.49$ & $9.52 \pm 0.17$ & $10.40 \pm 0.13$ & $10.80 \pm 0.11$ \\
NGC4151 & $-0.36 \pm 0.20$ & $8.92 \pm 0.18$ & $9.57 \pm 0.09$ & $9.98 \pm 0.06$ & $10.38 \pm 0.05$ \\
NGC4388 & $0.54 \pm 0.04$ & $8.75 \pm 0.13$ & $9.35 \pm 0.11$ & $10.51 \pm 0.09$ & $10.94 \pm 0.07$ \\
Mrk771 & $-0.28 \pm 1.89$ & $8.57 \pm 1.11$ & $9.62 \pm 0.12$ & $10.78 \pm 0.13$ & $11.17 \pm 0.12$ \\
NGC4941 & $-0.90 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $9.82 \pm 0.02$ & $10.22 \pm 0.02$ \\
MCG-03-34-064 & $0.33 \pm 0.29$ & $8.69 \pm 0.28$ & $9.34 \pm 0.20$ & $10.48 \pm 0.14$ & $10.91 \pm 0.11$ \\
ESO383-35 & $-1.15 \pm 0.26$ & $8.70 \pm 0.02$ & $9.54 \pm 0.06$ & $9.85 \pm 0.09$ & $10.25 \pm 0.08$ \\
ESO445-50 & $-1.28 \pm 0.53$ & $8.53 \pm 0.28$ & $9.67 \pm 0.07$ & $10.83 \pm 0.08$ & $11.21 \pm 0.07$ \\
NGC5506 & $-0.55 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.17 \pm 0.02$ & $10.57 \pm 0.02$ \\
2XMMJ141348.3+440014 & $1.06 \pm 0.20$ & $9.54 \pm 0.33$ & $8.91 \pm 0.53$ & $9.65 \pm 0.77$ & $10.13 \pm 0.61$ \\
NGC5548 & $0.14 \pm 0.32$ & $8.85 \pm 0.25$ & $9.59 \pm 0.08$ & $10.63 \pm 0.08$ & $11.03 \pm 0.07$ \\
Mrk1383 & $-0.16 \pm 1.13$ & $8.40 \pm 0.47$ & $9.60 \pm 0.13$ & $11.18 \pm 0.14$ & $11.57 \pm 0.12$ \\
Mrk841 & $1.04 \pm 0.02$ & $9.59 \pm 0.29$ & $9.01 \pm 0.14$ & $9.71 \pm 0.13$ & $10.22 \pm 0.11$ \\
ESO141-55 & $1.30 \pm 0.09$ & $9.61 \pm 0.29$ & $9.11 \pm 0.26$ & $10.18 \pm 0.45$ & $10.66 \pm 0.37$ \\
IC5063 & $-0.71 \pm 0.15$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.77 \pm 0.02$ & $11.16 \pm 0.02$ \\
Mrk1513 & $1.49 \pm 0.05$ & $9.60 \pm 0.28$ & $8.39 \pm 0.45$ & $9.41 \pm 0.75$ & $10.03 \pm 0.54$ \\
LEDA68751 & $0.66 \pm 0.18$ & $9.39 \pm 0.42$ & $9.22 \pm 0.30$ & $10.00 \pm 0.45$ & $10.44 \pm 0.41$ \\
NGC7674 & $1.45 \pm 0.04$ & $9.01 \pm 0.09$ & $9.36 \pm 0.03$ & $10.96 \pm 0.05$ & $11.40 \pm 0.04$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar2_LSM.tex <==
\begin{tabular}{cccccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
NGC0078 & $-0.21 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.50 \pm 0.02$ & $10.91 \pm 0.02$ \\
UM246 & $1.03 \pm 0.06$ & $9.00 \pm 0.20$ & $9.32 \pm 0.11$ & $10.47 \pm 0.09$ & $10.91 \pm 0.08$ \\
2MASXJ01221811+0100262 & $1.58 \pm 0.06$ & $9.69 \pm 0.21$ & $8.95 \pm 0.16$ & $10.12 \pm 0.13$ & $10.65 \pm 0.10$ \\
CGCG087-046 & $1.07 \pm 0.08$ & $8.84 \pm 0.15$ & $9.39 \pm 0.10$ & $11.00 \pm 0.05$ & $11.42 \pm 0.04$ \\
UGC04383 & $0.64 \pm 0.04$ & $8.70 \pm 0.08$ & $9.06 \pm 0.04$ & $9.82 \pm 0.02$ & $10.31 \pm 0.02$ \\
2MASXJ08343370+1720462 & $0.47 \pm 0.08$ & $8.91 \pm 0.13$ & $9.45 \pm 0.09$ & $10.40 \pm 0.07$ & $10.82 \pm 0.05$ \\
2MASXJ08381760+3054533 & $0.17 \pm 0.25$ & $8.77 \pm 0.14$ & $9.50 \pm 0.05$ & $10.77 \pm 0.02$ & $11.17 \pm 0.02$ \\
2MASXJ08434495+3549421 & $0.53 \pm 0.05$ & $8.92 \pm 0.12$ & $9.53 \pm 0.12$ & $10.71 \pm 0.11$ & $11.11 \pm 0.09$ \\
UGC05044 & $0.56 \pm 0.05$ & $8.84 \pm 0.15$ & $9.45 \pm 0.15$ & $10.64 \pm 0.12$ & $11.06 \pm 0.09$ \\
ARP142 & $0.75 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $11.03 \pm 0.02$ & $11.42 \pm 0.02$ \\
CGCG266-026 & $0.96 \pm 0.07$ & $8.99 \pm 0.05$ & $9.47 \pm 0.05$ & $10.81 \pm 0.07$ & $11.23 \pm 0.06$ \\
LSBCF567-01 & $-1.14 \pm 0.02$ & $9.64 \pm 0.19$ & $9.29 \pm 0.06$ & $7.86 \pm 0.05$ & $8.32 \pm 0.04$ \\
2MASXJ10225654+3446467 & $0.11 \pm 0.11$ & $8.70 \pm 0.05$ & $9.48 \pm 0.02$ & $10.82 \pm 0.02$ & $11.23 \pm 0.02$ \\
UGC05644 & $0.75 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $11.03 \pm 0.02$ & $11.42 \pm 0.02$ \\
CGCG037-076 & $1.22 \pm 0.03$ & $9.53 \pm 0.32$ & $8.57 \pm 0.10$ & $9.32 \pm 0.09$ & $9.93 \pm 0.07$ \\
UGCA219 & $-0.57 \pm 0.02$ & $9.10 \pm 0.37$ & $8.97 \pm 0.07$ & $8.15 \pm 0.04$ & $8.66 \pm 0.03$ \\
NGC3445 & $0.19 \pm 0.02$ & $9.57 \pm 0.30$ & $9.14 \pm 0.14$ & $9.02 \pm 0.10$ & $9.51 \pm 0.07$ \\
2MASXJ10591815+2432343 & $1.91 \pm 0.02$ & $9.28 \pm 0.55$ & $8.72 \pm 0.10$ & $10.28 \pm 0.04$ & $10.85 \pm 0.03$ \\
VV627 & $0.81 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $11.09 \pm 0.02$ & $11.49 \pm 0.02$ \\
IC0700 & $-0.86 \pm 0.02$ & $9.03 \pm 0.15$ & $9.20 \pm 0.05$ & $8.27 \pm 0.02$ & $8.74 \pm 0.02$ \\
UGC06665 & $1.13 \pm 0.04$ & $9.36 \pm 0.44$ & $8.61 \pm 0.09$ & $9.35 \pm 0.12$ & $9.94 \pm 0.10$ \\
UGC07388 & $0.19 \pm 0.08$ & $8.81 \pm 0.15$ & $9.37 \pm 0.09$ & $10.12 \pm 0.05$ & $10.54 \pm 0.04$ \\
NGC4320 & $0.36 \pm 0.08$ & $8.97 \pm 0.08$ & $9.57 \pm 0.09$ & $10.57 \pm 0.07$ & $10.97 \pm 0.06$ \\
UGC07936 & $0.60 \pm 0.07$ & $9.21 \pm 0.23$ & $9.37 \pm 0.11$ & $9.97 \pm 0.08$ & $10.41 \pm 0.07$ \\
MRK0237 & $1.00 \pm 0.03$ & $9.64 \pm 0.20$ & $9.30 \pm 0.07$ & $10.03 \pm 0.05$ & $10.49 \pm 0.04$ \\
UGC08327 & $1.12 \pm 0.10$ & $8.98 \pm 0.09$ & $9.36 \pm 0.06$ & $10.69 \pm 0.06$ & $11.12 \pm 0.05$ \\
UGC08335 & $1.92 \pm 0.07$ & $9.61 \pm 0.29$ & $8.66 \pm 0.14$ & $10.11 \pm 0.09$ & $10.70 \pm 0.07$ \\
NGC5100 & $0.94 \pm 0.08$ & $8.89 \pm 0.14$ & $9.42 \pm 0.09$ & $10.85 \pm 0.05$ & $11.28 \pm 0.04$ \\
CGCG017-018 & $1.04 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.56 \pm 0.02$ & $10.99 \pm 0.02$ \\
NGC5331 & $1.48 \pm 0.09$ & $8.86 \pm 0.18$ & $9.21 \pm 0.16$ & $10.81 \pm 0.11$ & $11.27 \pm 0.08$ \\
UGC09618 & $1.45 \pm 0.26$ & $8.65 \pm 0.43$ & $9.00 \pm 0.21$ & $10.75 \pm 0.07$ & $11.26 \pm 0.04$ \\
2MASXJ15015015+2332536 & $0.70 \pm 0.11$ & $8.98 \pm 0.07$ & $9.44 \pm 0.07$ & $10.48 \pm 0.09$ & $10.90 \pm 0.08$ \\
SBS1509+583 & $0.29 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $10.57 \pm 0.02$ & $10.97 \pm 0.02$ \\
KUG1553+200 & $1.23 \pm 0.02$ & $9.70 \pm 0.21$ & $9.16 \pm 0.11$ & $10.06 \pm 0.09$ & $10.54 \pm 0.07$ \\
KUG1556+326 & $0.66 \pm 0.08$ & $8.79 \pm 0.15$ & $9.36 \pm 0.09$ & $10.60 \pm 0.06$ & $11.03 \pm 0.04$ \\
MRK0881 & $0.94 \pm 0.03$ & $9.63 \pm 0.26$ & $9.09 \pm 0.10$ & $9.69 \pm 0.07$ & $10.19 \pm 0.05$ \\
2MASXJ17045097+3449020 & $1.59 \pm 0.02$ & $9.65 \pm 0.23$ & $9.23 \pm 0.10$ & $10.51 \pm 0.08$ & $10.99 \pm 0.06$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar2_SB.tex <==
\begin{tabular}{cccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
NGC23 & $0.91 \pm 0.06$ & $8.96 \pm 0.09$ & $9.47 \pm 0.06$ & $10.81 \pm 0.04$ & $11.23 \pm 0.04$ \\
NGC253 & $0.47 \pm 0.15$ & $8.92 \pm 0.12$ & $9.36 \pm 0.06$ & $10.14 \pm 0.06$ & $10.57 \pm 0.05$ \\
NGC660 & $0.10 \pm 0.13$ & $8.97 \pm 0.09$ & $9.49 \pm 0.09$ & $10.02 \pm 0.08$ & $10.44 \pm 0.06$ \\
NGC1222 & $0.82 \pm 0.02$ & $9.68 \pm 0.22$ & $9.08 \pm 0.09$ & $9.54 \pm 0.07$ & $10.05 \pm 0.05$ \\
NGC1365 & $1.14 \pm 0.14$ & $8.96 \pm 0.11$ & $9.39 \pm 0.10$ & $10.82 \pm 0.09$ & $11.25 \pm 0.07$ \\
IC342 & $-1.99 \pm 0.24$ & $8.84 \pm 0.15$ & $9.53 \pm 0.07$ & $8.49 \pm 0.02$ & $8.89 \pm 0.02$ \\
NGC1614 & $1.75 \pm 0.05$ & $9.60 \pm 0.27$ & $8.85 \pm 0.12$ & $10.19 \pm 0.08$ & $10.74 \pm 0.06$ \\
NGC1797 & $1.24 \pm 0.10$ & $9.68 \pm 0.22$ & $9.12 \pm 0.16$ & $9.99 \pm 0.12$ & $10.48 \pm 0.09$ \\
NGC2146 & $-0.42 \pm 0.80$ & $7.97 \pm 0.92$ & $8.69 \pm 0.35$ & $9.74 \pm 0.11$ & $10.30 \pm 0.06$ \\
NGC2623 & $1.29 \pm 0.05$ & $9.58 \pm 0.30$ & $9.00 \pm 0.09$ & $9.94 \pm 0.06$ & $10.45 \pm 0.04$ \\
NGC3256 & $1.72 \pm 0.02$ & $9.66 \pm 0.24$ & $9.09 \pm 0.09$ & $10.47 \pm 0.06$ & $10.97 \pm 0.05$ \\
NGC3310 & $0.56 \pm 0.03$ & $9.67 \pm 0.22$ & $8.93 \pm 0.10$ & $9.08 \pm 0.08$ & $9.61 \pm 0.06$ \\
NGC3556 & $0.00 \pm 0.08$ & $8.97 \pm 0.08$ & $9.47 \pm 0.06$ & $9.88 \pm 0.05$ & $10.29 \pm 0.04$ \\
NGC3628 & $-0.21 \pm 0.06$ & $8.70 \pm 0.03$ & $9.48 \pm 0.02$ & $10.51 \pm 0.02$ & $10.91 \pm 0.02$ \\
NGC4088 & $0.17 \pm 0.02$ & $8.99 \pm 0.06$ & $9.35 \pm 0.04$ & $9.68 \pm 0.04$ & $10.12 \pm 0.04$ \\
NGC4194 & $1.01 \pm 0.02$ & $9.42 \pm 0.39$ & $9.01 \pm 0.08$ & $9.73 \pm 0.04$ & $10.24 \pm 0.03$ \\
Mrk52 & $0.43 \pm 0.03$ & $9.59 \pm 0.19$ & $9.33 \pm 0.06$ & $9.52 \pm 0.04$ & $9.97 \pm 0.03$ \\
NGC4676 & $0.92 \pm 0.02$ & $9.00 \pm 0.03$ & $9.50 \pm 0.02$ & $10.82 \pm 0.02$ & $11.23 \pm 0.02$ \\
NGC4818 & $-0.16 \pm 0.09$ & $8.79 \pm 0.15$ & $9.36 \pm 0.09$ & $9.77 \pm 0.06$ & $10.20 \pm 0.05$ \\
NGC4945 & $1.22 \pm 0.25$ & $9.32 \pm 0.45$ & $9.23 \pm 0.21$ & $10.45 \pm 0.13$ & $10.91 \pm 0.09$ \\
NGC7252 & $0.76 \pm 0.03$ & $8.99 \pm 0.05$ & $9.49 \pm 0.04$ & $10.66 \pm 0.03$ & $11.07 \pm 0.02$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/CIGALEPar2_SIGS_stub.tex <==
\begin{tabular}{cccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
NGC275 & $0.11 \pm 0.06$ & $9.51 \pm 0.25$ & $9.31 \pm 0.09$ & $9.22 \pm 0.06$ & $9.67 \pm 0.05$ \\
NGC470 & $0.57 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.09 \pm 0.02$ & $10.53 \pm 0.02$ \\
NGC474 & $-0.36 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.35 \pm 0.02$ & $10.76 \pm 0.02$ \\
NGC520 & $0.35 \pm 0.15$ & $9.00 \pm 0.02$ & $9.58 \pm 0.05$ & $10.49 \pm 0.04$ & $10.89 \pm 0.04$ \\
IC196 & $-0.46 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.26 \pm 0.02$ & $10.67 \pm 0.02$ \\
NGC833 & $-1.16 \pm 0.17$ & $8.67 \pm 0.10$ & $9.61 \pm 0.04$ & $10.42 \pm 0.04$ & $10.81 \pm 0.04$ \\
NGC835 & $0.65 \pm 0.07$ & $8.86 \pm 0.15$ & $9.40 \pm 0.10$ & $10.57 \pm 0.05$ & $11.00 \pm 0.04$ \\
NGC838 & $0.99 \pm 0.04$ & $9.04 \pm 0.37$ & $9.18 \pm 0.11$ & $10.14 \pm 0.05$ & $10.61 \pm 0.04$ \\
NGC839 & $0.99 \pm 0.03$ & $9.42 \pm 0.25$ & $9.31 \pm 0.07$ & $10.12 \pm 0.03$ & $10.57 \pm 0.03$ \\
NGC935 & $0.62 \pm 0.03$ & $8.99 \pm 0.05$ & $9.49 \pm 0.03$ & $10.53 \pm 0.02$ & $10.94 \pm 0.02$ \\
IC1801 & $0.29 \pm 0.03$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.81 \pm 0.02$ & $10.25 \pm 0.02$ \\
NGC1241 & $0.62 \pm 0.05$ & $8.91 \pm 0.13$ & $9.52 \pm 0.13$ & $10.78 \pm 0.11$ & $11.18 \pm 0.09$ \\
NGC1242 & $-0.21 \pm 0.08$ & $8.99 \pm 0.05$ & $9.49 \pm 0.05$ & $9.67 \pm 0.05$ & $10.08 \pm 0.04$ \\
NGC1253 & $-0.10 \pm 0.23$ & $8.88 \pm 0.24$ & $9.38 \pm 0.21$ & $9.81 \pm 0.16$ & $10.24 \pm 0.13$ \\
NGC1253A & $-0.69 \pm 0.02$ & $8.94 \pm 0.38$ & $9.16 \pm 0.19$ & $8.52 \pm 0.09$ & $9.00 \pm 0.06$ \\
NGC2276 & $0.91 \pm 0.05$ & $9.40 \pm 0.26$ & $9.32 \pm 0.09$ & $10.06 \pm 0.06$ & $10.51 \pm 0.05$ \\
NGC2444 & $-1.28 \pm 0.09$ & $8.70 \pm 0.02$ & $9.61 \pm 0.03$ & $10.26 \pm 0.03$ & $10.65 \pm 0.03$ \\
NGC2445 & $0.76 \pm 0.04$ & $9.01 \pm 0.33$ & $9.20 \pm 0.18$ & $9.97 \pm 0.10$ & $10.44 \pm 0.07$ \\
NGC2633 & $0.84 \pm 0.02$ & $9.68 \pm 0.16$ & $9.33 \pm 0.06$ & $9.88 \pm 0.05$ & $10.34 \pm 0.04$ \\
NGC2634 & $-2.23 \pm 0.36$ & $8.69 \pm 0.07$ & $9.69 \pm 0.03$ & $9.94 \pm 0.04$ & $10.31 \pm 0.03$ \\
NGC2719A & $-0.08 \pm 0.02$ & $9.49 \pm 0.36$ & $8.79 \pm 0.10$ & $8.32 \pm 0.05$ & $8.88 \pm 0.03$ \\
NGC2719 & $-0.18 \pm 0.05$ & $8.86 \pm 0.25$ & $9.12 \pm 0.09$ & $8.99 \pm 0.04$ & $9.47 \pm 0.03$ \\
NGC2805 & $0.22 \pm 0.02$ & $8.75 \pm 0.25$ & $9.08 \pm 0.10$ & $9.41 \pm 0.04$ & $9.89 \pm 0.03$ \\
NGC2814 & $-0.68 \pm 0.06$ & $9.03 \pm 0.15$ & $9.36 \pm 0.05$ & $8.82 \pm 0.04$ & $9.25 \pm 0.03$ \\
NGC2820A & $-1.06 \pm 0.02$ & $9.33 \pm 0.41$ & $9.02 \pm 0.10$ & $7.67 \pm 0.06$ & $8.18 \pm 0.04$ \\
NGC2820 & $-0.16 \pm 0.04$ & $9.02 \pm 0.12$ & $9.36 \pm 0.03$ & $9.35 \pm 0.02$ & $9.79 \pm 0.02$ \\
NGC2964 & $0.23 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.75 \pm 0.02$ & $10.18 \pm 0.02$ \\
NGC2970 & $-2.41 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $9.09 \pm 0.02$ & $9.48 \pm 0.02$ \\
NGC2976 & $-1.13 \pm 0.04$ & $8.97 \pm 0.08$ & $9.48 \pm 0.05$ & $8.77 \pm 0.03$ & $9.19 \pm 0.02$ \\
NGC3031 & $-0.52 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.20 \pm 0.02$ & $10.61 \pm 0.02$ \\
NGC3034 & $-1.06 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $9.30 \pm 0.02$ & $9.87 \pm 0.02$ \\
NGC3077 & $-1.14 \pm 0.12$ & $8.85 \pm 0.17$ & $9.40 \pm 0.11$ & $8.80 \pm 0.07$ & $9.22 \pm 0.06$ \\
NGC3165 & $-1.23 \pm 0.05$ & $8.99 \pm 0.06$ & $9.49 \pm 0.05$ & $8.67 \pm 0.04$ & $9.09 \pm 0.03$ \\
NGC3166 & $-1.08 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.42 \pm 0.02$ & $10.81 \pm 0.02$ \\
NGC3169 & $-0.07 \pm 0.22$ & $8.87 \pm 0.15$ & $9.55 \pm 0.07$ & $10.37 \pm 0.02$ & $10.77 \pm 0.02$ \\
NGC3185 & $-0.67 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $9.61 \pm 0.02$ & $10.01 \pm 0.02$ \\
NGC3187 & $-0.42 \pm 0.02$ & $8.78 \pm 0.31$ & $9.09 \pm 0.13$ & $8.77 \pm 0.06$ & $9.26 \pm 0.04$ \\
NGC3190 & $-1.22 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.28 \pm 0.02$ & $10.67 \pm 0.02$ \\
NGC3226 & $-1.79 \pm 0.24$ & $8.63 \pm 0.17$ & $9.60 \pm 0.05$ & $9.84 \pm 0.05$ & $10.23 \pm 0.04$ \\
NGC3227 & $-0.17 \pm 0.02$ & $9.00 \pm 0.03$ & $9.61 \pm 0.03$ & $10.10 \pm 0.03$ & $10.49 \pm 0.03$ \\
NGC3395 & $0.31 \pm 0.02$ & $9.55 \pm 0.31$ & $9.07 \pm 0.09$ & $9.07 \pm 0.05$ & $9.57 \pm 0.04$ \\
NGC3396 & $0.24 \pm 0.02$ & $9.43 \pm 0.37$ & $9.05 \pm 0.11$ & $8.98 \pm 0.06$ & $9.49 \pm 0.04$ \\
NGC3424 & $0.13 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.65 \pm 0.02$ & $10.09 \pm 0.02$ \\
NGC3430 & $0.21 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.74 \pm 0.02$ & $10.17 \pm 0.02$ \\
NGC3448 & $-0.08 \pm 0.03$ & $8.75 \pm 0.24$ & $9.08 \pm 0.09$ & $9.10 \pm 0.04$ & $9.59 \pm 0.03$ \\
IC694 & $-1.96 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $8.40 \pm 0.02$ & $8.97 \pm 0.02$ \\
NGC3690 & $2.02 \pm 0.03$ & $9.12 \pm 0.59$ & $8.41 \pm 0.17$ & $9.95 \pm 0.18$ & $10.59 \pm 0.14$ \\
NGC3786 & $-0.10 \pm 0.02$ & $8.99 \pm 0.03$ & $9.60 \pm 0.03$ & $10.17 \pm 0.03$ & $10.57 \pm 0.03$ \\
NGC3788 & $-0.01 \pm 0.07$ & $8.98 \pm 0.07$ & $9.58 \pm 0.07$ & $10.20 \pm 0.08$ & $10.60 \pm 0.07$ \\
NGC3799 & $-0.09 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.43 \pm 0.02$ & $9.87 \pm 0.02$ \\
NGC3800 & $0.64 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.16 \pm 0.02$ & $10.59 \pm 0.02$ \\
IC749 & $-0.70 \pm 0.03$ & $8.97 \pm 0.08$ & $9.33 \pm 0.08$ & $8.78 \pm 0.08$ & $9.22 \pm 0.07$ \\
IC750 & $-0.61 \pm 0.05$ & $8.71 \pm 0.08$ & $9.32 \pm 0.05$ & $9.33 \pm 0.04$ & $9.77 \pm 0.04$ \\
NGC4038 & $1.08 \pm 0.03$ & $9.23 \pm 0.24$ & $9.33 \pm 0.16$ & $10.34 \pm 0.10$ & $10.79 \pm 0.07$ \\
NGC4394 & $-1.02 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $9.69 \pm 0.02$ & $10.10 \pm 0.02$ \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/LSMSample.tex <==
\begin{tabular}{ccrlrlcr}
\hline
Galaxy & RA & Dec\ \ \  & Redshift & $\log(L_{IR})$ & Stage & Size & Angle$^{\rm a}$\\
ID &\multicolumn{2}{c}{(J2000)} & \ \ \ ($z$) & ($L_{\odot}$)\ \ \  & &($\arcsec \times \arcsec$) & ($\degr$)\ \ \ \\
\hline
NGC 0078                & 00:20:26.6 &    00:49:46.7 & 0.0183 &  9.98 & 2.0 & $60.0  \times 35.0 $ & 145.0 \\
UM 246                  & 00:29:45.1 &    00:10:09.0 & 0.0594 & 10.83 & 4.5 & $60.0  \times 30.0 $ &  45.0 \\
2MASX J01221811+0100262 & 01:22:17.8 &    01:00:27.5 & 0.0555 & 11.54 & 4.0 & $39.0  \times 36.0 $ &  30.0 \\
CGCG 087-046            & 07:54:31.8 &    16:48:26.3 & 0.0463 & 11.28 & 4.0 & $45.0  \times 35.0 $ & 115.0 \\
UGC 04383               & 08:23:33.5 &    21:20:34.7 & 0.0179 & 10.46 & 3.0 & $55.0  \times 38.0 $ & 125.0 \\
2MASX J08343370+1720462 & 08:34:33.7 &    17:20:46.4 & 0.0479 & 10.86 & 4.0 & $30.0  \times 28.0 $ & 115.0 \\
2MASX J08381760+3054533 & 08:38:17.6 &    30:54:53.5 & 0.0477 & 10.62 & 4.0 & $28.0  \times 22.0 $ & 110.0 \\
2MASX J08434495+3549421 & 08:43:45.0 &    35:49:42.0 & 0.054  & 10.45 & 5.0 & $28.0  \times 25.0 $ &  55.0 \\
UGC 05044               & 09:27:44.0 &    12:17:12.3 & 0.029  & 10.52 & 4.0 & $50.0  \times 45.0 $ & 110.0 \\
Arp 142                 & 09:37:44.0 &    02:45:15.1 & 0.0233 & 10.89 & 3.5 & $65.0  \times 55.0 $ & 130.0 \\
CGCG 266-026            & 10:10:00.8 &    54:40:19.8 & 0.0462 & 10.91 & 4.5 & $50.0  \times 32.0 $ & 155.0 \\
LSBCF 567-01            & 10:19:01.5 &    21:17:01.3 & 0.0036 &  8.38 & 5.0 & $65.0  \times 35.0 $ &  65.0 \\
2MASX J10225654+3446467 & 10:22:56.6 &    34:46:46.8 & 0.0561 & 10.66 & 3.5 & $40.0  \times 32.0 $ &  65.0 \\
UGC 05644               & 10:25:46.3 &    13:43:00.7 & 0.0323 & 10.52 & 3.0 & $75.0  \times 32.0 $ & 130.0 \\
CGCG 037-076            & 10:33:28.6 &    07:08:03.8 & 0.0445 & 10.79 & 4.0 & $33.0  \times 28.0 $ &  70.0 \\
UGC A219                & 10:49:05.0 &    52:20:07.8 & 0.008  &  8.82 & 5.0 & $30.0  \times 25.0 $ &  60.0 \\
NGC 3445                & 10:54:35.5 &    56:59:26.5 & 0.0068 &  9.76 & 3.0 & $50.0  \times 45.0 $ &  70.0 \\
2MASX J10591815+2432343 & 10:59:18.1 &    24:32:34.5 & 0.0431 & 12.18 & 3.5 & $50.0  \times 42.0 $ &  20.0 \\
VV 627                  & 11:00:59.8 &    57:47:04.0 & 0.0477 & 10.60 & 4.0 & $70.0  \times 40.0 $ & 145.0 \\
IC 0700                 & 11:29:15.5 &    20:35:05.7 & 0.0049 &  8.57 & 5.0 & $55.0  \times 30.0 $ & 155.0 \\
UGC 06665               & 11:42:12.4 &    00:20:02.5 & 0.0186 & 10.83 & 5.0 & $60.0  \times 48.0 $ & 125.0 \\
UGC 07388               & 12:20:15.7 &    33:39:38.9 & 0.0215 & 10.52 & 5.0 & $40.0  \times 35.0 $ & 125.0 \\
NGC 4320                & 12:22:57.7 &    10:32:54.0 & 0.0267 & 10.55 & 4.5 & $60.0  \times 45.0 $ & 115.0 \\
UGC 07936               & 12:46:00.1 &    45:12:00.0 & 0.0247 & 10.23 & 4.0 & $65.0  \times 50.0 $ & 130.0 \\
Mrk 0237                & 13:01:17.6 &    48:03:38.0 & 0.0298 & 10.87 & 4.0 & $50.0  \times 38.0 $ &  30.0 \\
UGC 08327               & 13:15:15.6 &    44:24:26.0 & 0.0367 & 11.17 & 3.5 & $60.0  \times 42.0 $ &   0.0 \\
UGC 08335               & 13:15:33.1 &    62:07:30.4 & 0.0308 & 11.70 & 4.0 & $60.0  \times 35.0 $ &  35.0 \\
NGC 5100                & 13:20:58.6 &    08:58:55.0 & 0.0319 & 11.21 & 3.5 & $60.0  \times 50.0 $ &  50.0 \\
CGCG 017-018            & 13:32:55.9 & $-$03:01:37.0 & 0.0465 & 10.86 & 2.0 & $38.0  \times 25.0 $ &  20.0 \\
NGC 5331                & 13:52:16.3 &    02:06:10.9 & 0.033  & 11.23 & 3.0 & $65.0  \times 50.0 $ &  80.0 \\
CGCG 076-015$^{\rm b}$  
                        & 14:44:27.1 &    12:15:25.8 & 0.0528 & 10.96 & 4.0 & $23.0  \times 23.0 $ &   0.0 \\
UGC 09618               & 14:57:00.5 &    24:36:49.9 & 0.0329 & 11.26 & 2.0 & $60.0  \times 40.0 $ &  95.0 \\
2MASX J15015015+2332536 & 15:01:50.2 &    23:32:53.7 & 0.0463 & 10.92 & 4.5 & $32.0  \times 27.0 $ &  60.0 \\
SBS 1509+583            & 15:10:17.8 &    58:10:37.5 & 0.0319 & 10.37 & 2.0 & $35.0  \times 25.0 $ &  30.0 \\
KUG 1553+200            & 15:55:56.9 &    19:56:58.0 & 0.0413 & 11.00 & 4.0 & $32.0  \times 32.0 $ &   0.0 \\
KUG 1556+326            & 15:58:37.8 &    32:27:42.2 & 0.0482 & 10.76 & 3.0 & $38.0  \times 32.0 $ & 110.0 \\
Mrk 0881                & 16:25:49.4 &    40:20:42.7 & 0.0288 & 10.90 & 5.0 & $35.0  \times 30.0 $ &  95.0 \\
2MASX J17045097+3449020 & 17:04:50.9 &    34:49:02.4 & 0.0563 & 11.31 & 2.0 & $35.0  \times 30.0 $ &  40.0 \\
\hline
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/SBSample.tex <==
\begin{tabular}{ccrlccr}
\hline
Galaxy & RA & Dec\ \ \  & Redshift & Sample & Size & Angle$^{\rm a}$\\
ID &\multicolumn{2}{c}{(J2000)} & \ \ \ ($z$) & &($\arcsec \times \arcsec$) & ($\degr$)\ \ \ \\
\hline
NGC   23 & 00:09:53.4 &    25:55:25.6 & 0.0152 & S  &  86.3 $\times$  58.2 &  90.0 \\
NGC  253 & 00:47:32.4 & $-$25:17:44.0 & 0.0008 & S  & 820.4 $\times$ 226.5 & 140.0 \\
NGC  660 & 01:43:02.4 &    13:38:42.2 & 0.0028 & SB & 304.8 $\times$ 124.2 &  75.0 \\
NGC 1222 & 03:08:56.7 & $-$02:57:18.5 & 0.0081 & B  &  73.4 $\times$  60.0 &  70.0 \\
NGC 1365 & 03:33:36.4 & $-$36:08:28.2 & 0.0055 & B  & 353.8 $\times$ 221.6 & 128.0 \\
IC   342 & 03:46:48.5 &    68:05:46.9 & 0.0001 & B  & 716.5 $\times$ 598.5 &   0.0 \\
NGC 1614 & 04:33:59.8 & $-$08:34:44.0 & 0.0159 & B  &  82.9 $\times$  54.9 & 114.7 \\
NGC 1797 & 05:07:44.9 & $-$08:01:08.7 & 0.0149 & S  &  66.7 $\times$  41.0 & 162.9 \\
NGC 2146 & 06:18:37.7 &    78:21:25.3 & 0.003  & B  & 174.8 $\times$ 125.9 & 210.0 \\
NGC 2623 & 08:38:24.0 &    25:45:16.1 & 0.0185 & B  &  76.4 $\times$  45.8 & 160.0 \\
NGC 3256 & 10:27:51.3 & $-$43:54:13.5 & 0.0094 & SB & 224.4 $\times$ 135.8 &  10.0 \\
NGC 3310 & 10:38:45.9 &    53:30:12.2 & 0.0033 & B  & 126.4 $\times$ 104.4 &  93.3 \\
NGC 3556 & 11:11:31.0 &    55:40:26.8 & 0.0023 & B  & 262.2 $\times$  85.7 & 170.0 \\
NGC 3628 & 11:20:17.0 &    13:35:22.9 & 0.0028 & B  & 508.4 $\times$ 219.2 &  13.0 \\
NGC 4088 & 12:05:34.2 &    50:32:20.5 & 0.0025 & SB & 187.7 $\times$ 103.1 & 143.0 \\
NGC 4194 & 12:14:09.5 &    54:31:36.6 & 0.0083 & B  &  92.2 $\times$  53.4 &  90.0 \\
Mrk   52 & 12:25:42.8 &    00:34:21.4 & 0.0071 & B  &  62.7 $\times$  38.4 & 170.0 \\
NGC 4676 & 12:46:10.7 &    30:43:38.0 & 0.022  & B  & 155.1 $\times$  54.5 &  90.0 \\
NGC 4818 & 12:56:48.8 & $-$08:31:37.0 & 0.0036 & B  & 145.8 $\times$  66.0 &  90.0 \\
NGC 4945 & 13:05:27.5 & $-$49:28:05.6 & 0.0019 & SB & 571.9 $\times$ 150.0 & 133.0 \\
NGC 7252 & 22:20:44.7 & $-$24:40:41.7 & 0.016  & B  &  71.0 $\times$  62.7 &  80.0 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/SHLines.tex <==
\begin{tabular}{ccccccccc}
\hline
Galaxy ID & [\ion{Ne}{ii}] & [\ion{Ne}{iii}] & [\ion{Ne}{v}] & [\ion{S}{iii}] & [\ion{S}{iv}] & [\ion{Fe}{ii}] & H$_{2}$ S(2) & H$_{2}$ S(1)\\
&  12.81~\micron & 15.56~\micron & 14.32~\micron & 18.71~\micron & 10.51~\micron & 12.64~\micron & 12.28~\micron & 17.03~\micron \\
\hline
NGC 23 & 49.37$\pm$0.14 & 6.95$\pm$0.04 & $\cdots$ & 16.08$\pm$0.14 & 1.62$\pm$0.06 & 0.48$\pm$0.06 & 5.71$\pm$0.11 & 6.65$\pm$0.07 \\
NGC 253 & 2689.15$\pm$1.29 & 183.27$\pm$0.57 & $\cdots$ & 576.23$\pm$1.08 & $\cdots$ & 77.21$\pm$0.83 & 93.53$\pm$0.80 & 79.39$\pm$0.67 \\
NGC 520 & 46.18$\pm$0.21 & 6.84$\pm$0.09 & 0.23$\pm$0.08 & 6.71$\pm$0.11 & 0.13$\pm$0.09 & $\cdots$ & 5.24$\pm$0.12 & 8.89$\pm$0.10 \\
NGC 660 & 286.20$\pm$0.34 & 27.60$\pm$0.19 & 1.30$\pm$0.14 & 54.78$\pm$0.24 & 1.47$\pm$0.22 & 3.40$\pm$0.14 & 6.30$\pm$0.13 & 17.82$\pm$0.20 \\
NGC 1222 & 82.21$\pm$0.16 & 78.18$\pm$0.13 & 0.47$\pm$0.06 & 49.33$\pm$0.17 & 25.16$\pm$0.12 & 0.69$\pm$0.09 & 4.79$\pm$0.09 & 7.92$\pm$0.08 \\
NGC 1365 & 178.44$\pm$0.37 & 55.36$\pm$0.23 & 18.74$\pm$0.20 & 55.25$\pm$0.30 & 28.31$\pm$0.29 & 4.35$\pm$0.17 & 12.61$\pm$0.18 & 20.18$\pm$0.18 \\
IC 342 & 639.63$\pm$0.38 & 34.58$\pm$0.16 & 2.31$\pm$0.16 & 255.47$\pm$0.39 & 5.20$\pm$0.21 & 11.80$\pm$0.21 & 12.01$\pm$0.26 & 9.30$\pm$0.18 \\
NGC 1614 & 265.07$\pm$0.30 & 66.59$\pm$0.19 & 1.63$\pm$0.10 & 70.91$\pm$0.30 & 11.65$\pm$0.17 & 1.97$\pm$0.14 & 6.84$\pm$0.15 & 10.05$\pm$0.14 \\
NGC 1797 & 67.82$\pm$0.19 & 5.33$\pm$0.07 & 0.34$\pm$0.12 & 18.63$\pm$0.16 & 1.11$\pm$0.09 & 0.53$\pm$0.10 & 3.50$\pm$0.14 & 3.92$\pm$0.10 \\
NGC 2146 & 803.04$\pm$1.52 & 121.59$\pm$0.43 & 2.99$\pm$0.31 & 253.62$\pm$1.17 & 21.55$\pm$0.82 & 10.90$\pm$0.30 & 10.07$\pm$0.28 & 37.91$\pm$0.35 \\
NGC 2623 & 73.10$\pm$0.57 & 20.68$\pm$0.26 & 3.54$\pm$0.11 & 13.55$\pm$0.32 & 7.31$\pm$0.42 & 1.31$\pm$0.21 & 5.51$\pm$0.17 & 14.12$\pm$0.31 \\
NGC 3256 & 495.57$\pm$0.50 & 61.04$\pm$0.18 & 0.92$\pm$0.15 & 138.36$\pm$0.35 & 10.49$\pm$0.17 & 8.29$\pm$0.20 & 20.34$\pm$0.17 & 26.12$\pm$0.16 \\
NGC 3310 & 43.45$\pm$0.22 & 28.62$\pm$0.15 & 0.25$\pm$0.10 & 19.36$\pm$0.26 & 5.56$\pm$0.15 & 0.46$\pm$0.09 & 0.84$\pm$0.16 & 2.04$\pm$0.13 \\
NGC 3556 & 21.51$\pm$0.10 & 3.01$\pm$0.05 & 0.06$\pm$0.06 & 10.28$\pm$0.12 & 0.42$\pm$0.10 & 0.24$\pm$0.08 & 1.67$\pm$0.12 & 2.46$\pm$0.06 \\
NGC 3628 & 170.98$\pm$0.66 & 13.28$\pm$0.12 & 0.69$\pm$0.09 & 32.91$\pm$0.31 & $\cdots$ & 2.92$\pm$0.18 & 10.02$\pm$0.21 & 28.46$\pm$0.29 \\
NGC 4088 & 35.01$\pm$0.14 & 2.24$\pm$0.06 & 0.43$\pm$0.16 & 9.31$\pm$0.08 & 0.28$\pm$0.13 & 0.28$\pm$0.06 & 2.45$\pm$0.09 & 3.97$\pm$0.06 \\
NGC 4194 & 162.22$\pm$0.26 & 50.57$\pm$0.17 & 1.99$\pm$0.09 & 56.92$\pm$0.22 & 15.11$\pm$0.21 & 2.50$\pm$0.14 & 6.63$\pm$0.15 & 7.26$\pm$0.13 \\
Mrk 52 & 24.39$\pm$0.09 & 3.34$\pm$0.07 & $\cdots$ & 17.71$\pm$0.09 & 1.11$\pm$0.07 & 0.41$\pm$0.06 & 1.00$\pm$0.06 & 1.54$\pm$0.07 \\
NGC 4676 & 34.68$\pm$0.23 & 6.87$\pm$0.12 & 0.44$\pm$0.05 & 16.18$\pm$0.22 & 2.63$\pm$0.20 & 0.65$\pm$0.08 & 3.07$\pm$0.09 & 8.86$\pm$0.15 \\
NGC 4818 & 154.06$\pm$0.22 & 11.12$\pm$0.12 & 0.97$\pm$0.12 & 47.40$\pm$0.24 & 2.35$\pm$0.10 & 4.34$\pm$0.17 & 6.11$\pm$0.32 & 13.59$\pm$0.15 \\
NGC 4945 & 978.73$\pm$2.18 & 114.10$\pm$0.49 & 9.49$\pm$0.27 & 106.69$\pm$0.77 & 31.63$\pm$2.62 & 17.47$\pm$0.50 & 80.48$\pm$0.50 & 228.37$\pm$1.41 \\
NGC 7252 & 36.31$\pm$0.13 & 2.99$\pm$0.06 & 0.34$\pm$0.06 & 8.28$\pm$0.09 & 0.12$\pm$0.07 & 0.08$\pm$0.05 & 3.12$\pm$0.13 & 3.56$\pm$0.07 \\
NGC 7714 & 94.55$\pm$0.17 & 63.77$\pm$0.11 & $\cdots$ & 56.86$\pm$0.14 & 16.38$\pm$0.15 & 2.26$\pm$0.11 & 3.44$\pm$0.10 & 3.19$\pm$0.09 \\
\hline
\end{tabular}

==> QuantifiyingAGN_arXiv 2/Tables/SIGSSample.tex <==
\newcommand{\0}{\phantom{0}}
\begin{tabular}{cccrlcccr}
\hline
Group & Galaxy & RA & Dec\ \ \  & Redshift & Sample & Interaction & Size & Angle$^{\rm a}$\\
 ID   & ID &\multicolumn{2}{c}{(J2000)} & \ \ \ ($z$) &&Stage&($\arcsec \times \arcsec$) & ($\degr$)\ \ \ \\
\hline
\01 & NGC 274$^{\rm b}$
                & 00:51:01.6 & $-$07:03:22.7 & 0.0058 & A & 4 &  33.8  $\times$  23.0 & 130.0 \\
    & NGC 275   & 00:51:04.8 & $-$07:03:59.8 & 0.0058 & A & 4 &  38.2  $\times$  28.1 &  25.0 \\
\02 & NGC 470   & 01:19:44.9 &    03:24:35.6 & 0.0079 & A & 2 &  90.0  $\times$  55.1 &  65.0 \\
    & NGC 474   & 01:20:06.7 &    03:24:55.4 & 0.0077 & A & 2 & 225.0  $\times$ 175.0 & 165.0 \\
\03 & NGC 520   & 01:24:35.1 &    03:47:32.7 & 0.0076 & A & 5 & 147.3  $\times$  97.2 & 235.0 \\
\04 &  IC 195$^{\rm b}$   & 02:03:44.6 &    14:42:33.5 & 0.0122 & A & 3 &  37.8  $\times$  21.2 &  39.8 \\
    &  IC 196   & 02:03:49.8 &    14:44:20.8 & 0.0122 & A & 3 &  95.0  $\times$  55.1 &  62.0 \\
\05 & NGC 833   & 02:09:20.8 & $-$10:07:59.2 & 0.0129 & A & 4 &  42.5  $\times$  23.0 & 175.0 \\
    & NGC 835   & 02:09:24.6 & $-$10:08:09.2 & 0.0136 & A & 4 &  42.8  $\times$  35.3 & 125.0 \\
    & NGC 838   & 02:09:38.5 & $-$10:08:48.1 & 0.0128 & A & 3 &  45.0  $\times$  25.9 & 175.0 \\
    & NGC 839   & 02:09:42.9 & $-$10:11:02.8 & 0.0129 & A & 2 &  45.0  $\times$  28.0 &   5.0 \\
\06 & NGC 935   & 02:28:10.6 &    19:36:05.4 & 0.0138 & A & 4 &  53.6  $\times$  33.1 &  65.0 \\
    & IC 1801   & 02:28:12.7 &    19:34:59.9 & 0.0134 & A & 4 &  34.2  $\times$  19.1 & 120.0 \\
\07 & NGC 1241  & 03:11:14.6 & $-$08:55:19.6 & 0.0135 & A & 3 & 100.1  $\times$  60.1 &  50.0 \\
    & NGC 1242  & 03:11:19.3 & $-$08:54:08.6 & 0.0134 & A & 3 &  28.1  $\times$  19.4 &  44.4 \\
\08 & NGC 1253  & 03:14:09.0 & $-$02:49:22.4 & 0.0057 & A & 3 & 168.1  $\times$  52.6 & 175.0 \\
    & NGC 1253A & 03:14:23.3 & $-$02:48:02.9 & 0.0061 & A & 3 &  55.1  $\times$  20.2 &   5.0 \\
\09 & NGC 2276  & 07:27:28.3 &    85:45:23.8 & 0.0081 & C & 2 &  85.0  $\times$  72.0 & 110.0 \\
 10 & NGC 2444  & 07:46:53.2 &    39:02:05.3 & 0.0135 & A & 4 &  54.4  $\times$  30.6 & 125.0 \\
    & NGC 2445  & 07:46:55.1 &    39:00:41.8 & 0.0133 & A & 4 &  52.2  $\times$  45.4 & 110.0 \\
 11 & NGC 2633  & 08:48:04.6 &    74:05:56.0 & 0.0072 & C & 2 &  79.9  $\times$  50.0 &  90.0 \\
    & NGC 2634$^{\rm b}$
                & 08:48:25.4 &    73:58:01.9 & 0.0075 & C & 2 &  40.7  $\times$  35.3 & 135.0 \\
    & NGC 2634A & 08:48:38.1 &    73:56:21.5 & 0.007  & C & 2 &  38.2  $\times$  18.0 & 155.0 \\
 12 & NGC 2719A & 09:00:15.5 &    35:43:09.5 & 0.0104 & A & 2 &  22.0  $\times$  15.1 &  35.0 \\
    & NGC 2719  & 09:00:15.6 &    35:43:41.9 & 0.0103 & A & 2 &  40.0  $\times$  13.0 &  40.0 \\
 13 & NGC 2805  & 09:20:20.4 &    64:06:10.1 & 0.0058 & C & 2 & 165.0  $\times$ 140.0 & 120.0 \\
    & NGC 2814  & 09:21:11.5 &    64:15:11.5 & 0.0053 & C & 2 &  50.0  $\times$  20.2 &  90.0 \\
 14 & NGC 2820A & 09:21:29.8 &    64:14:14.6 & 0.0051 & C & 3 &  15.5  $\times$  11.2 & 110.0 \\
    & NGC 2820  & 09:21:45.6 &    64:15:28.4 & 0.0053 & C & 3 & 119.9  $\times$  20.2 & 151.0 \\
 15 & NGC 2964  & 09:42:54.2 &    31:50:50.6 & 0.0044 & C & 2 &  78.5  $\times$  41.0 &   8.0 \\
    & NGC 2968$^{\rm b}$  & 09:43:12.0 &    31:55:43.3 & 0.0052 & C & 2 &  71.3  $\times$  54.4 & 145.0 \\
    & NGC 2970  & 09:43:31.1 &    31:58:37.2 & 0.0054 & C & 2 &  24.8  $\times$  24.8 &   0.0 \\
 16 & NGC 2976  & 09:47:15.5 &    67:54:59.0 & 0.0008 & C & 2 & 209.2  $\times$  84.6 &  50.6 \\
 17 & NGC 3031  & 09:55:33.2 &    69:03:55.1 & 0.0008 & C & 2 & 834.8  $\times$ 420.1 &  75.0 \\
    & NGC 3034  & 09:55:52.7 &    69:40:45.8 & 0.0007 & C & 2 & 285.1  $\times$ 159.8 & 155.0 \\
    & NGC 3077  & 10:03:19.1 &    68:44:02.0 & 0.0009 & C & 2 & 143.6  $\times$ 110.0 & 135.0 \\
 18 & NGC 3165  & 10:13:31.3 &    03:22:30.0 & 0.0045 & C & 3 &  70.9  $\times$  30.2 &  78.5 \\
    & NGC 3166  & 10:13:45.8 &    03:25:30.0 & 0.0045 & C & 3 & 141.1  $\times$  68.8 & 175.0 \\
    & NGC 3169  & 10:14:15.0 &    03:27:58.0 & 0.0041 & C & 2 & 150.1  $\times$ 110.2 & 145.0 \\
 19 & NGC 3185  & 10:17:38.6 &    21:41:17.9 & 0.0041 & C & 2 &  79.9  $\times$  55.1 &  35.0 \\
    & NGC 3187  & 10:17:47.9 &    21:52:23.9 & 0.0053 & C & 3 &  90.0  $\times$  40.0 & 170.0 \\
    & NGC 3190  & 10:18:05.6 &    21:49:56.3 & 0.0042 & C & 3 & 141.8  $\times$  50.0 &  32.0 \\
 20 & NGC 3226  & 10:23:27.0 &    19:53:54.6 & 0.0044 & C & 4 &  56.9  $\times$  44.6 & 110.0 \\
    & NGC 3227  & 10:23:30.6 &    19:51:54.0 & 0.0039 & C & 4 &  95.0  $\times$  60.1 &  55.0 \\
 21 & NGC 3395  & 10:49:49.3 &    32:58:45.5 & 0.0054 & C & 4 &  55.1  $\times$  32.0 & 120.0 \\
    & NGC 3396  & 10:49:55.6 &    32:59:24.7 & 0.0054 & C & 4 &  63.0  $\times$  29.9 &  10.0 \\
 22 & NGC 3424  & 10:51:46.3 &    32:54:02.9 & 0.005  & C & 2 &  93.6  $\times$  28.8 &  20.0 \\
    & NGC 3430  & 10:52:11.4 &    32:57:01.4 & 0.0053 & C & 2 & 119.2  $\times$  69.1 & 115.0 \\
 23 & UGC 6016$^{\rm b}$
                & 10:54:14.6 &    54:17:11.8 & 0.005  & A & 3 &  74.9  $\times$  47.9 & 150.0 \\
    & NGC 3448  & 10:54:38.6 &    54:18:22.3 & 0.0045 & A & 3 &  84.6  $\times$  40.3 & 155.0 \\
 24 &   IC 694  & 11:28:27.3 &    58:34:42.6 & 0.0132 & C & 4 &  11.9  $\times$  11.9 &   0.0 \\
    & NGC 3690  & 11:28:32.3 &    58:33:42.8 & 0.0104 & C & 4 &  65.9  $\times$  47.2 &  35.0 \\
 25 & NGC 3786  & 11:39:42.7 &    31:54:27.7 & 0.0089 & C & 3 &  62.3  $\times$  33.5 & 170.0 \\
    & NGC 3788  & 11:39:44.6 &    31:55:52.3 & 0.009  & C & 3 &  58.0  $\times$  25.9 &  85.0 \\
 26 & NGC 3799  & 11:40:09.4 &    15:19:38.3 & 0.011  & A & 3 &  25.2  $\times$  18.4 &  14.2 \\
    & NGC 3800  & 11:40:13.5 &    15:20:32.6 & 0.011  & A & 3 &  61.2  $\times$  24.5 & 142.0 \\
 27 &   IC 749  & 11:58:34.1 &    42:44:02.4 & 0.0027 & C & 2 &  79.9  $\times$  65.2 &  65.0 \\
    &   IC 750  & 11:58:52.2 &    42:43:21.0 & 0.0023 & C & 2 &  79.9  $\times$  45.4 & 130.0 \\
 28 & NGC 4038  & 12:01:54.3 & $-$18:53:03.1 & 0.0055 & A & 4 & 142.9  $\times$ 107.6 &  84.3 \\
 29 & NGC 4382$^{\rm b}$  & 12:25:24.1 &    18:11:29.4 & 0.0024 & C & 2 & 150.1  $\times$ 114.8 &  95.0 \\
    & NGC 4394  & 12:25:55.5 &    18:12:50.8 & 0.0031 & C & 2 & 110.2  $\times$  95.0 &  15.0 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/SIGSSample2.tex <==
\begin{tabular}{cccrlcccr}
\hline
Group & Galaxy & RA & Dec\ \ \  & Redshift & Sample & Interaction & Size & Angle$^{\rm a}$\\
 ID   & ID &\multicolumn{2}{c}{(J2000)} & \ \ \ ($z$) &&Stage&($\arcsec \times \arcsec$) & ($\degr$)\ \ \ \\
\hline
30 & NGC 4567  & 12:36:31.5 &    11:15:43.6 & 0.0075 & C & 3 &  72.0  $\times$  43.2 & 145.0 \\
   & NGC 4568  & 12:36:34.5 &    11:14:12.5 & 0.0075 & C & 3 & 142.9  $\times$  41.8 & 122.0 \\
31 & NGC 4618  & 12:41:32.9 &    41:08:42.4 & 0.0018 & C & 3 & 135.0  $\times$ 105.1 & 115.0 \\
   & NGC 4625  & 12:41:52.7 &    41:16:26.4 & 0.0021 & C & 3 &  65.5  $\times$  57.2 &  56.7 \\
32 & NGC 4647  & 12:43:31.7 &    11:35:03.5 & 0.0047 & C & 3 &  68.0  $\times$  55.1 &  20.0 \\
   & NGC 4649  & 12:43:40.0 &    11:33:09.7 & 0.0037 & C & 3 & 119.9  $\times$  95.0 &  10.0 \\
33 & NGC 4933A$^{\rm b}$ & 13:03:53.9 & $-$11:30:23.8 & 0.0104 & A & 4 &  24.8  $\times$  20.2 & 155.0 \\
   & NGC 4933B & 13:03:57.2 & $-$11:29:43.8 & 0.0108 & A & 4 &  40.0  $\times$  38.2 & 130.0 \\
   & NGC 4933C & 13:04:01.1 & $-$11:29:26.2 & 0.0106 & A & 4 &  15.8  $\times$  14.0 &  20.0 \\
34 & M51A      & 13:29:51.6 &    47:10:34.7 & 0.0015 & C & 3 & 273.2  $\times$ 204.0 & 120.0 \\
   & M51B      & 13:29:59.6 &    47:15:58.0 & 0.0016 & C & 3 & 107.6  $\times$  65.5 &   5.0 \\
35 & NGC 5350  & 13:53:21.6 &    40:21:50.0 & 0.0077 & C & 3 & 100.1  $\times$  69.8 & 125.0 \\
35 & NGC 5353  & 13:53:26.7 &    40:16:58.8 & 0.0078 & C & 3 &  52.9  $\times$  28.1 &  52.0 \\
   & NGC 5354  & 13:53:26.7 &    40:18:10.1 & 0.0086 & C & 2 &  42.1  $\times$  36.0 &   0.0 \\
36 & NGC 5394  & 13:58:32.4 &    37:27:14.8 & 0.0115 & C & 4 &  50.0  $\times$  45.0 & 110.0 \\
   & NGC 5395  & 13:58:38.0 &    37:25:28.2 & 0.0117 & C & 4 &  92.2  $\times$  50.4 &  87.2 \\
37 & NGC 5457  & 14:03:12.5 &    54:20:56.4 & 0.0008 & C & 3 & 650.2  $\times$ 650.0 &   0.0 \\
   & NGC 5474  & 14:05:01.6 &    53:39:43.9 & 0.0009 & C & 3 & 142.6  $\times$ 124.0 & 282.5 \\
38 & NGC 5426  & 14:03:24.8 & $-$06:04:08.8 & 0.0086 & A & 4 &  79.9  $\times$  51.8 &  75.0 \\
   & NGC 5427  & 14:03:26.0 & $-$06:01:50.9 & 0.0087 & A & 4 &  77.0  $\times$  61.9 &   0.0 \\
39 & NGC 5480  & 14:06:21.6 &    50:43:30.4 & 0.0062 & C & 2 &  62.6  $\times$  50.0 &  85.0 \\
   & NGC 5481  & 14:06:41.3 &    50:43:23.9 & 0.0066 & C & 2 &  60.1  $\times$  42.1 &  15.0 \\
40 & NGC 5544  & 14:17:03.0 &    36:34:19.6 & 0.0101 & C & 3 &  69.8  $\times$  42.1 & 150.0 \\
41 & NGC 5614  & 14:24:07.6 &    34:51:31.7 & 0.013  & C & 4 &  79.2  $\times$  45.4 &  45.0 \\
42 & NGC 5846$^{\rm b}$  & 15:06:29.3 &    01:36:20.2 & 0.0057 & C & 2 &  92.2  $\times$  81.4 & 125.0 \\
   & NGC 5850  & 15:07:07.7 &    01:32:39.1 & 0.0085 & C & 2 & 138.0  $\times$ 110.0 &  10.0 \\
43 & NGC 5905  & 15:15:23.3 &    55:31:02.6 & 0.0113 & C & 3 & 160.0  $\times$  75.0 &  38.0 \\
   & NGC 5908  & 15:16:43.2 &    55:24:33.5 & 0.011  & C & 2 &  83.5  $\times$  41.8 &  63.2 \\
44 & NGC 5929  & 15:26:05.4 &    41:40:07.3 & 0.0083 & C & 4 &  22.7  $\times$  20.2 & 130.0 \\
   & NGC 5930  & 15:26:08.2 &    41:40:44.0 & 0.0087 & C & 4 &  67.0  $\times$  23.4 &  70.0 \\
45 & NGC 5953  & 15:34:31.9 &    15:11:38.8 & 0.0066 & A & 4 &  31.0  $\times$  28.1 & 160.0 \\
   & NGC 5954  & 15:34:34.8 &    15:12:05.8 & 0.0065 & A & 4 &  38.5  $\times$  20.9 &  90.0 \\
46 & NGC 5981  & 15:37:53.4 &    59:23:30.5 & 0.0059 & C & 2 &  95.0  $\times$  15.5 &  49.2 \\
   & NGC 5985  & 15:39:37.1 &    59:19:54.8 & 0.0084 & C & 2 & 169.9  $\times$  82.1 & 110.0 \\
47 & Arp 314A  & 22:58:02.2 & $-$03:46:10.9 & 0.0123 & A & 4 &  34.9  $\times$  28.1 & 115.0 \\
   & Arp 314C$^{\rm b}$
               & 22:58:07.4 & $-$03:48:41.4 & 0.0123 & A & 4 &  38.2  $\times$  31.0 &  70.0 \\
   & Arp 314B  & 22:58:07.9 & $-$03:47:19.7 & 0.0124 & A & 4 &  34.9  $\times$  32.0 &  90.0 \\
48 & NGC 7715  & 23:36:22.1 &    02:09:23.4 & 0.0092 & A & 4 &  52.9  $\times$  23.4 & 160.0 \\
   & NGC 7714  & 23:36:14.1 &    02:09:18.6 & 0.0093 & A & 4 &  81.7  $\times$  53.3 & 155.0 \\
\hline
\end{tabular}


==> QuantifiyingAGN_arXiv 2/Tables/SeptKS.tex <==
\begin{tabular}{cccccccccccc}
\hline
Samples & $f_{\rm{AGN}}$ & L(AGN) & E$(B-V)$ & E$(B-V)$ & $\alpha$ & L(dust) & SFR & age(stars) & Mgas & M$_*$ & sSFR \\
Compared & & & (Old Stars) & (Young Stars)& (Dust) \\
\hline
2-3 & 0.44 & 0.42 & 0.95 & 0.96 & 0.24 & 0.88 & 0.91 & 0.62 & 0.59 & 0.92 & 0.24 \\
2-4 & 0.3 & 0.05 & 0.01 & 0.01 & 0.38 & <0.01 & 0.01 & 0.07 & 0.42 & 0.26 & 0.5 \\
2-5 & 0.12 & 0.01 & 0.03 & 0.03 & 0.34 & 0.02 & 0.05 & 0.75 & 0.49 & 0.49 & 0.07 \\
2-AGN & <0.01 & <0.01 & <0.01 & 0.66 & <0.01 & 0.02 & 0.84 & 0.19 & <0.01 & <0.01 & 0.09 \\
3-4 & 0.43 & 0.18 & <0.01 & 0.01 & <0.01 & 0.01 & 0.02 & 0.26 & 0.63 & 0.49 & 0.1 \\
3-5 & 0.21 & 0.02 & 0.03 & 0.08 & 0.06 & 0.05 & 0.17 & 0.8 & 0.22 & 0.22 & 0.14 \\
3-AGN & <0.01 & <0.01 & <0.01 & 0.86 & <0.01 & <0.01 & 0.76 & 0.03 & <0.01 & <0.01 & <0.01 \\
4-5 & 0.61 & 0.42 & 0.51 & 0.97 & 0.84 & 0.83 & 0.98 & 0.92 & 0.51 & 0.51 & 0.38 \\
4-AGN & <0.01 & <0.01 & 0.31 & 0.06 & 0.08 & 0.43 & 0.10 & 0.01 & 0.01 & 0.04 & <0.01 \\
5-AGN & <0.01 & 0.02 & 0.56 & 0.15 & 0.38 & 0.56 & 0.15 & 0.17 & 0.07 & 0.07 & <0.01 \\
SB-2 & 0.31 & 0.03 & 0.01 & 0.01 & 0.11 & <0.01 & 0.01 & 0.2 & 0.43 & 0.41 & 0.05 \\
SB-3 & 0.61 & 0.05 & <0.01 & 0.01 & <0.01 & <0.01 & 0.02 & 0.44 & 0.35 & 0.35 & 0.1 \\
SB-4 & >0.99 & 0.85 & 0.22 & 0.43 & 0.42 & 0.43 & 0.43 & 0.76 & 0.98 & 0.99 & 0.18 \\
SB-5 & 0.53 & 0.38 & 0.08 & 0.64 & 0.93 & 0.26 & 0.48 & 0.85 & 0.58 & 0.64 & 0.96 \\
SB-AGN & <0.01 & <0.01 & 0.07 & 0.01 & 0.60 & 0.07 & 0.04 & 0.03 & 0.04 & 0.09 & <0.01 \\
noAGN-AGN & <0.01 & 0.01 & 0.18 & 0.03 & <0.01 & 0.28 & 0.04 & 0.01 & 0.02 & 0.02 & <0.01 \\
\hline
\end{tabular}	


==> QuantifiyingAGN_arXiv 2/Tables/par_cig.tex <==
\begin{tabular}{p{0.15\textwidth}p{0.25\textwidth}p{0.45\textwidth}}
\hline
\hline
Parameter & Values & Description \\
\hline
\multicolumn{3}{c}{Star formation history (SFH): Delayed}\\
$\tau_{\textnormal{main}}$&50, 500, 1000, 2500, 5000, 7500& e-folding time of the main stellar population model (Myr).\\
Age &500, 1000, 2000, 3000, 4000, 5000, 6000&Age of the oldest stars in the galaxy (Myr).\\
\hline
\multicolumn{3}{c}{Single-age stellar population (SSP): \citet{2003MNRAS.344.1000B}}\\
Separation Age& 10& Age of the separation (to differentiate) between the young and the old star populations (Myr).\\
\hline
\multicolumn{3}{c}{Dust attenuation: \citet{2000ApJ...533..682C}}\\
E$(B-V)_{\textnormal{young}}$ &0.1, 0.25, 0.4, 0.55, 0.7& Color excess of the stellar continuum light for the young population.\\
E$(B-V)_{\textnormal{old factor}}$ &0.22, 0.44, 0.66, 0.88 & Reduction factor for the  E$(B-V)$ of the old population compared to the young one.\\
Power-law slope ($\delta$) & 0.0, 0.25, 0.5& Slope delta of the power law modifying the attenuation curve.\\
\hline
\multicolumn{3}{c}{Dust emission: \citet{2014ApJ...784...83D}}\\
$\alpha$ & 1.0, 1.25, 1.5, 1.75, 2.0, 2.25, 2.5, 2.75, 3.0 & Alpha from the power-law distribution in eq.~\ref{eq:alpha}. \\
\hline
\multicolumn{3}{c}{AGN model: \citet{2006MNRAS.366..767F}}\\
R$_{\textnormal{max}}$/R$_{\textnormal{min}}$ & 10.0, 30.0, 60.0, 100.0, 150.0 & Ratio of the maximum to minimum radii of the dust torus. \\
$\tau$ & 0.1, 0.6, 1.0, 6.0, 10.0 & Optical depth at 9.7 $\micron$. \\
$\beta$ & $-$1.00, $-$0.75, $-$0.50, $-$0.25, 0.00 & Beta from the power-law density distribution for the radial component of the dust torus (eq. 3 of Fritz 2006).\\
$\gamma$ & 0.0, 2.0 & Gamma from the power-law density distribution for the polar component of the dust torus (eq. 3 of Fritz 2006).\\
Opening Angle ($\theta$) & 60.0, 100.0, 140.0 & Full opening angle of the dust torus (Fig 1 of Fritz 2006). \\
$\psi$ & 30.1$^{\rm a}$ & Angle between equatorial axis and line of sight. \\
$f_{\rm{AGN}}$ & 0.1 -- 0.9 in steps of 0.05 & Fraction of AGN torus contribution to the IR luminosity (fracAGN in Equ. 1 of Ciesla 2015)\\
\hline
\end{tabular}


==> Tables/CIGALEPar1_SIGS.tex <==
\begin{tabular}{ccccccc}
\hline
Galaxy &$f_{\rm{AGN}}$ & $L_{\rm{AGN}}$ & Old Att. & Young Att. &Dust $\alpha$ & $L_{\rm{dust}}$ \\
ID&&$\log(L_\odot)$&$\log(L_\odot)$& $\log(L_\odot)$&&$\log(L_\odot)$ \\
\hline
NGC275 & 0.20 $\pm$ 0.14 & $9.26 \pm 0.30$ & $9.42 \pm 0.09$ & $9.57 \pm 0.07$ & 2.09 $\pm$ 0.18 & $9.84 \pm 0.07$ \\
NGC470 & $\cdots$ & $\cdots$ & $10.22 \pm 0.02$ & $10.04 \pm 0.03$ & 2.00 $\pm$ 0.10 & $10.47 \pm 0.02$ \\
NGC474 & $\cdots$ & $\cdots$ & $9.65 \pm 0.05$ & $8.94 \pm 0.06$ & 2.04 $\pm$ 0.10 & $9.74 \pm 0.04$ \\
NGC520 & 0.58 $\pm$ 0.08 & $10.69 \pm 0.07$ & $10.45 \pm 0.06$ & $9.81 \pm 0.16$ & 2.37 $\pm$ 0.28 & $10.56 \pm 0.08$ \\
IC196 & $\cdots$ & $\cdots$ & $9.66 \pm 0.02$ & $8.82 \pm 0.02$ & 2.32 $\pm$ 0.12 & $9.73 \pm 0.02$ \\
NGC833 & 0.27 $\pm$ 0.07 & $9.09 \pm 0.15$ & $9.50 \pm 0.02$ & $8.11 \pm 0.17$ & 2.87 $\pm$ 0.17 & $9.52 \pm 0.02$ \\
NGC835 & $\cdots$ & $\cdots$ & $10.60 \pm 0.04$ & $10.12 \pm 0.07$ & 2.00 $\pm$ 0.10 & $10.74 \pm 0.02$ \\
NGC838 & $\cdots$ & $\cdots$ & $10.71 \pm 0.02$ & $10.48 \pm 0.04$ & 1.75 $\pm$ 0.09 & $10.94 \pm 0.02$ \\
NGC839 & $\cdots$ & $\cdots$ & $10.70 \pm 0.02$ & $10.48 \pm 0.03$ & 1.50 $\pm$ 0.07 & $10.93 \pm 0.02$ \\
NGC935 & $\cdots$ & $\cdots$ & $10.54 \pm 0.02$ & $10.11 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.70 \pm 0.02$ \\
IC1801 & $\cdots$ & $\cdots$ & $10.06 \pm 0.02$ & $9.77 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.27 \pm 0.02$ \\
NGC1241 & 0.21 $\pm$ 0.09 & $10.13 \pm 0.18$ & $10.57 \pm 0.05$ & $10.09 \pm 0.07$ & 2.54 $\pm$ 0.27 & $10.71 \pm 0.05$ \\
NGC1242 & 0.41 $\pm$ 0.08 & $9.44 \pm 0.09$ & $9.40 \pm 0.07$ & $9.09 \pm 0.14$ & 2.68 $\pm$ 0.23 & $9.60 \pm 0.05$ \\
NGC1253 & 0.21 $\pm$ 0.09 & $9.20 \pm 0.18$ & $9.61 \pm 0.14$ & $9.19 \pm 0.22$ & 2.57 $\pm$ 0.27 & $9.77 \pm 0.05$ \\
NGC1253A & $\cdots$ & $\cdots$ & $8.22 \pm 0.03$ & $8.58 \pm 0.02$ & 1.75 $\pm$ 0.09 & $8.79 \pm 0.02$ \\
NGC2276 & 0.20 $\pm$ 0.08 & $10.13 \pm 0.18$ & $10.40 \pm 0.06$ & $10.38 \pm 0.06$ & 2.44 $\pm$ 0.24 & $10.73 \pm 0.04$ \\
NGC2444 & $\cdots$ & $\cdots$ & $9.05 \pm 0.02$ & $8.00 \pm 0.09$ & 2.00 $\pm$ 0.10 & $9.10 \pm 0.02$ \\
NGC2445 & $\cdots$ & $\cdots$ & $10.28 \pm 0.05$ & $10.24 \pm 0.05$ & 1.97 $\pm$ 0.10 & $10.59 \pm 0.02$ \\
NGC2633 & $\cdots$ & $\cdots$ & $10.40 \pm 0.02$ & $10.32 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.70 \pm 0.02$ \\
NGC2634 & $\cdots$ & $\cdots$ & $8.64 \pm 0.02$ & $7.04 \pm 0.36$ & 2.96 $\pm$ 0.15 & $8.65 \pm 0.02$ \\
NGC2719A & $\cdots$ & $\cdots$ & $8.65 \pm 0.06$ & $9.19 \pm 0.02$ & 1.50 $\pm$ 0.07 & $9.35 \pm 0.02$ \\
NGC2719 & 0.26 $\pm$ 0.11 & $8.88 \pm 0.22$ & $8.80 \pm 0.14$ & $9.10 \pm 0.05$ & 1.88 $\pm$ 0.13 & $9.32 \pm 0.07$ \\
NGC2805 & $\cdots$ & $\cdots$ & $9.38 \pm 0.04$ & $9.51 \pm 0.02$ & 2.47 $\pm$ 0.12 & $9.79 \pm 0.02$ \\
NGC2814 & 0.42 $\pm$ 0.11 & $8.86 \pm 0.12$ & $8.69 \pm 0.08$ & $8.63 \pm 0.13$ & 2.54 $\pm$ 0.30 & $8.99 \pm 0.08$ \\
NGC2820A & $\cdots$ & $\cdots$ & $7.69 \pm 0.02$ & $8.21 \pm 0.02$ & 1.69 $\pm$ 0.11 & $8.37 \pm 0.02$ \\
NGC2820 & 0.25 $\pm$ 0.07 & $9.24 \pm 0.13$ & $9.46 \pm 0.04$ & $9.29 \pm 0.05$ & 2.47 $\pm$ 0.20 & $9.72 \pm 0.04$ \\
NGC2964 & 0.22 $\pm$ 0.08 & $9.57 \pm 0.16$ & $9.82 \pm 0.06$ & $9.71 \pm 0.03$ & 2.23 $\pm$ 0.16 & $10.10 \pm 0.04$ \\
NGC2970 & $\cdots$ & $\cdots$ & $7.89 \pm 0.02$ & $6.86 \pm 0.02$ & 1.17 $\pm$ 0.18 & $7.94 \pm 0.02$ \\
NGC2976 & 0.29 $\pm$ 0.04 & $8.32 \pm 0.06$ & $8.42 \pm 0.05$ & $8.31 \pm 0.05$ & 2.91 $\pm$ 0.15 & $8.70 \pm 0.03$ \\
NGC3031 & $\cdots$ & $\cdots$ & $9.46 \pm 0.02$ & $8.76 \pm 0.02$ & 2.96 $\pm$ 0.15 & $9.55 \pm 0.02$ \\
NGC3034 & 0.48 $\pm$ 0.03 & $10.19 \pm 0.05$ & $10.20 \pm 0.02$ & $8.46 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.21 \pm 0.02$ \\
NGC3077 & 0.30 $\pm$ 0.07 & $8.30 \pm 0.11$ & $8.45 \pm 0.09$ & $8.18 \pm 0.11$ & 2.00 $\pm$ 0.10 & $8.66 \pm 0.03$ \\
NGC3165 & $\cdots$ & $\cdots$ & $7.86 \pm 0.09$ & $8.04 \pm 0.05$ & 2.01 $\pm$ 0.10 & $8.30 \pm 0.02$ \\
NGC3166 & 0.21 $\pm$ 0.04 & $9.06 \pm 0.09$ & $9.60 \pm 0.02$ & $8.36 \pm 0.02$ & 2.56 $\pm$ 0.14 & $9.63 \pm 0.02$ \\
NGC3169 & $\cdots$ & $\cdots$ & $10.04 \pm 0.06$ & $9.38 \pm 0.27$ & 2.71 $\pm$ 0.19 & $10.14 \pm 0.03$ \\
NGC3185 & $\cdots$ & $\cdots$ & $9.12 \pm 0.02$ & $8.81 \pm 0.02$ & 2.25 $\pm$ 0.11 & $9.32 \pm 0.02$ \\
NGC3187 & 0.21 $\pm$ 0.05 & $8.64 \pm 0.11$ & $8.91 \pm 0.04$ & $8.86 \pm 0.02$ & 2.95 $\pm$ 0.15 & $9.22 \pm 0.02$ \\
NGC3190 & $\cdots$ & $\cdots$ & $9.73 \pm 0.02$ & $8.22 \pm 0.03$ & 2.50 $\pm$ 0.13 & $9.74 \pm 0.02$ \\
NGC3226 & $\cdots$ & $\cdots$ & $8.79 \pm 0.02$ & $7.49 \pm 0.24$ & 2.26 $\pm$ 0.11 & $8.82 \pm 0.02$ \\
NGC3227 & 0.20 $\pm$ 0.03 & $9.32 \pm 0.08$ & $9.76 \pm 0.04$ & $9.30 \pm 0.03$ & 2.26 $\pm$ 0.11 & $9.91 \pm 0.02$ \\
NGC3395 & $\cdots$ & $\cdots$ & $9.52 \pm 0.08$ & $9.65 \pm 0.07$ & 2.00 $\pm$ 0.10 & $9.93 \pm 0.02$ \\
NGC3396 & $\cdots$ & $\cdots$ & $9.52 \pm 0.04$ & $9.70 \pm 0.02$ & 1.75 $\pm$ 0.09 & $9.96 \pm 0.02$ \\
NGC3424 & $\cdots$ & $\cdots$ & $9.89 \pm 0.02$ & $9.62 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.10 \pm 0.02$ \\
NGC3430 & $\cdots$ & $\cdots$ & $9.61 \pm 0.03$ & $9.67 \pm 0.02$ & 2.39 $\pm$ 0.12 & $9.98 \pm 0.02$ \\
NGC3448 & 0.40 $\pm$ 0.05 & $9.46 \pm 0.07$ & $9.20 \pm 0.05$ & $9.36 \pm 0.04$ & 2.27 $\pm$ 0.11 & $9.63 \pm 0.03$ \\
IC694 & $\cdots$ & $\cdots$ & $9.02 \pm 0.06$ & $7.54 \pm 0.03$ & 1.24 $\pm$ 0.19 & $9.03 \pm 0.06$ \\
NGC3690 & $\cdots$ & $\cdots$ & $11.47 \pm 0.02$ & $11.51 \pm 0.03$ & 1.25 $\pm$ 0.06 & $11.83 \pm 0.02$ \\
NGC3786 & 0.22 $\pm$ 0.08 & $9.39 \pm 0.16$ & $9.75 \pm 0.05$ & $9.36 \pm 0.03$ & 2.22 $\pm$ 0.11 & $9.92 \pm 0.04$ \\
NGC3788 & $\cdots$ & $\cdots$ & $9.86 \pm 0.02$ & $9.45 \pm 0.07$ & 2.29 $\pm$ 0.11 & $10.02 \pm 0.02$ \\
NGC3799 & $\cdots$ & $\cdots$ & $9.27 \pm 0.08$ & $9.26 \pm 0.08$ & 2.25 $\pm$ 0.11 & $9.60 \pm 0.02$ \\
NGC3800 & $\cdots$ & $\cdots$ & $10.36 \pm 0.03$ & $10.09 \pm 0.02$ & 2.23 $\pm$ 0.11 & $10.57 \pm 0.02$ \\
IC749 & $\cdots$ & $\cdots$ & $8.61 \pm 0.05$ & $8.74 \pm 0.04$ & 2.25 $\pm$ 0.11 & $9.02 \pm 0.02$ \\
IC750 & 0.33 $\pm$ 0.07 & $9.32 \pm 0.11$ & $9.52 \pm 0.04$ & $8.88 \pm 0.04$ & 2.65 $\pm$ 0.26 & $9.62 \pm 0.04$ \\
NGC4038 & $\cdots$ & $\cdots$ & $10.61 \pm 0.04$ & $10.55 \pm 0.04$ & 2.00 $\pm$ 0.10 & $10.91 \pm 0.02$ \\
NGC4394 & $\cdots$ & $\cdots$ & $9.08 \pm 0.03$ & $8.26 \pm 0.02$ & 2.59 $\pm$ 0.21 & $9.15 \pm 0.02$ \\
NGC4567 & $\cdots$ & $\cdots$ & $10.03 \pm 0.04$ & $9.92 \pm 0.05$ & 2.25 $\pm$ 0.11 & $10.32 \pm 0.02$ \\
NGC4568 & $\cdots$ & $\cdots$ & $10.69 \pm 0.02$ & $10.37 \pm 0.05$ & 2.25 $\pm$ 0.11 & $10.88 \pm 0.02$ \\
NGC4618 & $\cdots$ & $\cdots$ & $8.65 \pm 0.09$ & $8.83 \pm 0.02$ & 2.26 $\pm$ 0.11 & $9.09 \pm 0.02$ \\
NGC4625 & $\cdots$ & $\cdots$ & $8.31 \pm 0.06$ & $8.41 \pm 0.05$ & 2.25 $\pm$ 0.11 & $8.71 \pm 0.02$ \\
NGC4647 & $\cdots$ & $\cdots$ & $9.77 \pm 0.02$ & $9.69 \pm 0.02$ & 2.25 $\pm$ 0.11 & $10.06 \pm 0.02$ \\
NGC4649 & $\cdots$ & $\cdots$ & $9.42 \pm 0.02$ & $7.69 \pm 0.08$ & 2.69 $\pm$ 0.18 & $9.43 \pm 0.02$ \\
NGC4933B & $\cdots$ & $\cdots$ & $9.64 \pm 0.02$ & $8.25 \pm 0.18$ & 2.66 $\pm$ 0.17 & $9.66 \pm 0.02$ \\
NGC4933C & $\cdots$ & $\cdots$ & $8.25 \pm 0.26$ & $7.98 \pm 0.26$ & 2.48 $\pm$ 0.36 & $8.46 \pm 0.08$ \\
M51A & $\cdots$ & $\cdots$ & $10.04 \pm 0.03$ & $9.96 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.34 \pm 0.02$ \\
M51B & 0.30 $\pm$ 0.16 & $8.74 \pm 0.23$ & $9.08 \pm 0.09$ & $7.52 \pm 0.03$ & 2.23 $\pm$ 0.24 & $9.10 \pm 0.09$ \\
NGC5350 & $\cdots$ & $\cdots$ & $10.08 \pm 0.06$ & $9.65 \pm 0.12$ & 2.48 $\pm$ 0.12 & $10.24 \pm 0.02$ \\
NGC5353 & $\cdots$ & $\cdots$ & $9.29 \pm 0.02$ & $5.54 \pm 4.46$ & 2.50 $\pm$ 0.12 & $9.29 \pm 0.02$ \\
NGC5354 & $\cdots$ & $\cdots$ & $9.14 \pm 0.02$ & $7.40 \pm 0.08$ & 2.25 $\pm$ 0.11 & $9.15 \pm 0.02$ \\
NGC5394 & $\cdots$ & $\cdots$ & $10.39 \pm 0.04$ & $10.24 \pm 0.03$ & 1.75 $\pm$ 0.09 & $10.66 \pm 0.02$ \\
NGC5395 & $\cdots$ & $\cdots$ & $10.47 \pm 0.04$ & $10.19 \pm 0.07$ & 2.47 $\pm$ 0.12 & $10.68 \pm 0.02$ \\
NGC5457 & $\cdots$ & $\cdots$ & $9.43 \pm 0.05$ & $9.36 \pm 0.05$ & 2.46 $\pm$ 0.12 & $9.73 \pm 0.02$ \\
NGC5426 & $\cdots$ & $\cdots$ & $10.21 \pm 0.13$ & $9.62 \pm 0.42$ & 2.27 $\pm$ 0.11 & $10.32 \pm 0.02$ \\
NGC5427 & $\cdots$ & $\cdots$ & $10.36 \pm 0.14$ & $10.22 \pm 0.19$ & 2.25 $\pm$ 0.11 & $10.63 \pm 0.02$ \\
NGC5474 & 0.34 $\pm$ 0.02 & $7.60 \pm 0.04$ & $7.85 \pm 0.02$ & $6.76 \pm 0.02$ & 2.93 $\pm$ 0.15 & $7.88 \pm 0.02$ \\
NGC5480 & $\cdots$ & $\cdots$ & $9.71 \pm 0.06$ & $9.74 \pm 0.05$ & 2.25 $\pm$ 0.11 & $10.06 \pm 0.02$ \\
NGC5481 & $\cdots$ & $\cdots$ & $8.66 \pm 0.02$ & $6.40 \pm 1.23$ & 1.08 $\pm$ 0.13 & $8.67 \pm 0.02$ \\
NGC5544 & $\cdots$ & $\cdots$ & $9.64 \pm 0.02$ & $9.34 \pm 0.02$ & 2.28 $\pm$ 0.11 & $9.84 \pm 0.02$ \\
NGC5614 & $\cdots$ & $\cdots$ & $10.32 \pm 0.03$ & $9.48 \pm 0.02$ & 2.49 $\pm$ 0.12 & $10.39 \pm 0.02$ \\
NGC5850 & $\cdots$ & $\cdots$ & $9.90 \pm 0.03$ & $9.14 \pm 0.02$ & 2.92 $\pm$ 0.15 & $9.98 \pm 0.02$ \\
NGC5905 & $\cdots$ & $\cdots$ & $10.14 \pm 0.06$ & $10.21 \pm 0.03$ & 2.25 $\pm$ 0.11 & $10.52 \pm 0.02$ \\
NGC5908 & $\cdots$ & $\cdots$ & $10.67 \pm 0.02$ & $9.56 \pm 0.12$ & 2.28 $\pm$ 0.11 & $10.71 \pm 0.02$ \\
NGC5929 & 0.40 $\pm$ 0.14 & $9.24 \pm 0.22$ & $9.32 \pm 0.09$ & $8.40 \pm 0.09$ & 1.85 $\pm$ 0.25 & $9.38 \pm 0.09$ \\
NGC5930 & 0.38 $\pm$ 0.24 & $10.14 \pm 0.27$ & $10.27 \pm 0.23$ & $9.39 \pm 0.33$ & 2.17 $\pm$ 0.44 & $10.33 \pm 0.17$ \\
NGC5953 & $\cdots$ & $\cdots$ & $10.30 \pm 0.02$ & $8.60 \pm 0.02$ & 2.00 $\pm$ 0.10 & $10.31 \pm 0.02$ \\
NGC5954 & $\cdots$ & $\cdots$ & $9.73 \pm 0.03$ & $9.66 \pm 0.03$ & 2.00 $\pm$ 0.10 & $10.04 \pm 0.02$ \\
NGC5981 & $\cdots$ & $\cdots$ & $9.34 \pm 0.02$ & $7.61 \pm 0.04$ & 2.72 $\pm$ 0.17 & $9.35 \pm 0.02$ \\
NGC5985 & $\cdots$ & $\cdots$ & $10.07 \pm 0.07$ & $9.72 \pm 0.11$ & 2.92 $\pm$ 0.15 & $10.25 \pm 0.02$ \\
ARP314A & 0.25 $\pm$ 0.11 & $9.94 \pm 0.20$ & $10.08 \pm 0.05$ & $10.04 \pm 0.06$ & 2.03 $\pm$ 0.11 & $10.40 \pm 0.05$ \\
ARP314B & $\cdots$ & $\cdots$ & $9.81 \pm 0.03$ & $9.83 \pm 0.02$ & 1.75 $\pm$ 0.09 & $10.16 \pm 0.02$ \\
NGC7714 & $\cdots$ & $\cdots$ & $10.37 \pm 0.02$ & $10.41 \pm 0.02$ & 1.50 $\pm$ 0.08 & $10.73 \pm 0.02$ \\
NGC7715 & $\cdots$ & $\cdots$ & $8.60 \pm 0.13$ & $7.90 \pm 0.91$ & 2.14 $\pm$ 0.45 & $8.69 \pm 0.19$ \\
\hline
\end{tabular}


==> Tables/CIGALEPar2_SIGS.tex <==
\begin{tabular}{cccccc}
\hline
Galaxy &  SFR & $\tau_{\rm{main}}$ & Stellar Age & $M_{\rm{gas}}$ & $M_{\star}$ \\
ID& $\log(M_\odot /yr)$ & $\log(yr)$ & $\log(yr)$ & $\log(M_\odot)$& $\log(M_\odot)$\\
\hline
NGC275 & $0.11 \pm 0.06$ & $9.51 \pm 0.25$ & $9.31 \pm 0.09$ & $9.22 \pm 0.06$ & $9.67 \pm 0.05$ \\
NGC470 & $0.57 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.09 \pm 0.02$ & $10.53 \pm 0.02$ \\
NGC474 & $-0.36 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.35 \pm 0.02$ & $10.76 \pm 0.02$ \\
NGC520 & $0.35 \pm 0.15$ & $9.00 \pm 0.02$ & $9.58 \pm 0.05$ & $10.49 \pm 0.04$ & $10.89 \pm 0.04$ \\
IC196 & $-0.46 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.26 \pm 0.02$ & $10.67 \pm 0.02$ \\
NGC833 & $-1.16 \pm 0.17$ & $8.67 \pm 0.10$ & $9.61 \pm 0.04$ & $10.42 \pm 0.04$ & $10.81 \pm 0.04$ \\
NGC835 & $0.65 \pm 0.07$ & $8.86 \pm 0.15$ & $9.40 \pm 0.10$ & $10.57 \pm 0.05$ & $11.00 \pm 0.04$ \\
NGC838 & $0.99 \pm 0.04$ & $9.04 \pm 0.37$ & $9.18 \pm 0.11$ & $10.14 \pm 0.05$ & $10.61 \pm 0.04$ \\
NGC839 & $0.99 \pm 0.03$ & $9.42 \pm 0.25$ & $9.31 \pm 0.07$ & $10.12 \pm 0.03$ & $10.57 \pm 0.03$ \\
NGC935 & $0.62 \pm 0.03$ & $8.99 \pm 0.05$ & $9.49 \pm 0.03$ & $10.53 \pm 0.02$ & $10.94 \pm 0.02$ \\
IC1801 & $0.29 \pm 0.03$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.81 \pm 0.02$ & $10.25 \pm 0.02$ \\
NGC1241 & $0.62 \pm 0.05$ & $8.91 \pm 0.13$ & $9.52 \pm 0.13$ & $10.78 \pm 0.11$ & $11.18 \pm 0.09$ \\
NGC1242 & $-0.21 \pm 0.08$ & $8.99 \pm 0.05$ & $9.49 \pm 0.05$ & $9.67 \pm 0.05$ & $10.08 \pm 0.04$ \\
NGC1253 & $-0.10 \pm 0.23$ & $8.88 \pm 0.24$ & $9.38 \pm 0.21$ & $9.81 \pm 0.16$ & $10.24 \pm 0.13$ \\
NGC1253A & $-0.69 \pm 0.02$ & $8.94 \pm 0.38$ & $9.16 \pm 0.19$ & $8.52 \pm 0.09$ & $9.00 \pm 0.06$ \\
NGC2276 & $0.91 \pm 0.05$ & $9.40 \pm 0.26$ & $9.32 \pm 0.09$ & $10.06 \pm 0.06$ & $10.51 \pm 0.05$ \\
NGC2444 & $-1.28 \pm 0.09$ & $8.70 \pm 0.02$ & $9.61 \pm 0.03$ & $10.26 \pm 0.03$ & $10.65 \pm 0.03$ \\
NGC2445 & $0.76 \pm 0.04$ & $9.01 \pm 0.33$ & $9.20 \pm 0.18$ & $9.97 \pm 0.10$ & $10.44 \pm 0.07$ \\
NGC2633 & $0.84 \pm 0.02$ & $9.68 \pm 0.16$ & $9.33 \pm 0.06$ & $9.88 \pm 0.05$ & $10.34 \pm 0.04$ \\
NGC2634 & $-2.23 \pm 0.36$ & $8.69 \pm 0.07$ & $9.69 \pm 0.03$ & $9.94 \pm 0.04$ & $10.31 \pm 0.03$ \\
NGC2719A & $-0.08 \pm 0.02$ & $9.49 \pm 0.36$ & $8.79 \pm 0.10$ & $8.32 \pm 0.05$ & $8.88 \pm 0.03$ \\
NGC2719 & $-0.18 \pm 0.05$ & $8.86 \pm 0.25$ & $9.12 \pm 0.09$ & $8.99 \pm 0.04$ & $9.47 \pm 0.03$ \\
NGC2805 & $0.22 \pm 0.02$ & $8.75 \pm 0.25$ & $9.08 \pm 0.10$ & $9.41 \pm 0.04$ & $9.89 \pm 0.03$ \\
NGC2814 & $-0.68 \pm 0.06$ & $9.03 \pm 0.15$ & $9.36 \pm 0.05$ & $8.82 \pm 0.04$ & $9.25 \pm 0.03$ \\
NGC2820A & $-1.06 \pm 0.02$ & $9.33 \pm 0.41$ & $9.02 \pm 0.10$ & $7.67 \pm 0.06$ & $8.18 \pm 0.04$ \\
NGC2820 & $-0.16 \pm 0.04$ & $9.02 \pm 0.12$ & $9.36 \pm 0.03$ & $9.35 \pm 0.02$ & $9.79 \pm 0.02$ \\
NGC2964 & $0.23 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.75 \pm 0.02$ & $10.18 \pm 0.02$ \\
NGC2970 & $-2.41 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $9.09 \pm 0.02$ & $9.48 \pm 0.02$ \\
NGC2976 & $-1.13 \pm 0.04$ & $8.97 \pm 0.08$ & $9.48 \pm 0.05$ & $8.77 \pm 0.03$ & $9.19 \pm 0.02$ \\
NGC3031 & $-0.52 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.20 \pm 0.02$ & $10.61 \pm 0.02$ \\
NGC3034 & $-1.06 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $9.30 \pm 0.02$ & $9.87 \pm 0.02$ \\
NGC3077 & $-1.14 \pm 0.12$ & $8.85 \pm 0.17$ & $9.40 \pm 0.11$ & $8.80 \pm 0.07$ & $9.22 \pm 0.06$ \\
NGC3165 & $-1.23 \pm 0.05$ & $8.99 \pm 0.06$ & $9.49 \pm 0.05$ & $8.67 \pm 0.04$ & $9.09 \pm 0.03$ \\
NGC3166 & $-1.08 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.42 \pm 0.02$ & $10.81 \pm 0.02$ \\
NGC3169 & $-0.07 \pm 0.22$ & $8.87 \pm 0.15$ & $9.55 \pm 0.07$ & $10.37 \pm 0.02$ & $10.77 \pm 0.02$ \\
NGC3185 & $-0.67 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $9.61 \pm 0.02$ & $10.01 \pm 0.02$ \\
NGC3187 & $-0.42 \pm 0.02$ & $8.78 \pm 0.31$ & $9.09 \pm 0.13$ & $8.77 \pm 0.06$ & $9.26 \pm 0.04$ \\
NGC3190 & $-1.22 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $10.28 \pm 0.02$ & $10.67 \pm 0.02$ \\
NGC3226 & $-1.79 \pm 0.24$ & $8.63 \pm 0.17$ & $9.60 \pm 0.05$ & $9.84 \pm 0.05$ & $10.23 \pm 0.04$ \\
NGC3227 & $-0.17 \pm 0.02$ & $9.00 \pm 0.03$ & $9.61 \pm 0.03$ & $10.10 \pm 0.03$ & $10.49 \pm 0.03$ \\
NGC3395 & $0.31 \pm 0.02$ & $9.55 \pm 0.31$ & $9.07 \pm 0.09$ & $9.07 \pm 0.05$ & $9.57 \pm 0.04$ \\
NGC3396 & $0.24 \pm 0.02$ & $9.43 \pm 0.37$ & $9.05 \pm 0.11$ & $8.98 \pm 0.06$ & $9.49 \pm 0.04$ \\
NGC3424 & $0.13 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.65 \pm 0.02$ & $10.09 \pm 0.02$ \\
NGC3430 & $0.21 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.74 \pm 0.02$ & $10.17 \pm 0.02$ \\
NGC3448 & $-0.08 \pm 0.03$ & $8.75 \pm 0.24$ & $9.08 \pm 0.09$ & $9.10 \pm 0.04$ & $9.59 \pm 0.03$ \\
IC694 & $-1.96 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $8.40 \pm 0.02$ & $8.97 \pm 0.02$ \\
NGC3690 & $2.02 \pm 0.03$ & $9.12 \pm 0.59$ & $8.41 \pm 0.17$ & $9.95 \pm 0.18$ & $10.59 \pm 0.14$ \\
NGC3786 & $-0.10 \pm 0.02$ & $8.99 \pm 0.03$ & $9.60 \pm 0.03$ & $10.17 \pm 0.03$ & $10.57 \pm 0.03$ \\
NGC3788 & $-0.01 \pm 0.07$ & $8.98 \pm 0.07$ & $9.58 \pm 0.07$ & $10.20 \pm 0.08$ & $10.60 \pm 0.07$ \\
NGC3799 & $-0.09 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.43 \pm 0.02$ & $9.87 \pm 0.02$ \\
NGC3800 & $0.64 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.16 \pm 0.02$ & $10.59 \pm 0.02$ \\
IC749 & $-0.70 \pm 0.03$ & $8.97 \pm 0.08$ & $9.33 \pm 0.08$ & $8.78 \pm 0.08$ & $9.22 \pm 0.07$ \\
IC750 & $-0.61 \pm 0.05$ & $8.71 \pm 0.08$ & $9.32 \pm 0.05$ & $9.33 \pm 0.04$ & $9.77 \pm 0.04$ \\
NGC4038 & $1.08 \pm 0.03$ & $9.23 \pm 0.24$ & $9.33 \pm 0.16$ & $10.34 \pm 0.10$ & $10.79 \pm 0.07$ \\
NGC4394 & $-1.02 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $9.69 \pm 0.02$ & $10.10 \pm 0.02$ \\
NGC4567 & $0.49 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $10.01 \pm 0.02$ & $10.45 \pm 0.02$ \\
NGC4568 & $0.93 \pm 0.06$ & $9.00 \pm 0.02$ & $9.39 \pm 0.06$ & $10.52 \pm 0.09$ & $10.95 \pm 0.08$ \\
NGC4618 & $-0.44 \pm 0.02$ & $8.72 \pm 0.17$ & $9.07 \pm 0.07$ & $8.74 \pm 0.03$ & $9.23 \pm 0.02$ \\
NGC4625 & $-1.01 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $8.52 \pm 0.02$ & $8.95 \pm 0.02$ \\
NGC4647 & $0.20 \pm 0.02$ & $9.00 \pm 0.02$ & $9.36 \pm 0.02$ & $9.72 \pm 0.02$ & $10.16 \pm 0.02$ \\
NGC4649 & $-1.59 \pm 0.08$ & $8.69 \pm 0.07$ & $9.70 \pm 0.02$ & $10.73 \pm 0.02$ & $11.11 \pm 0.02$ \\
NGC4933B & $-1.03 \pm 0.18$ & $8.64 \pm 0.16$ & $9.58 \pm 0.06$ & $10.53 \pm 0.05$ & $10.92 \pm 0.04$ \\
NGC4933C & $-1.30 \pm 0.26$ & $8.81 \pm 0.29$ & $9.33 \pm 0.26$ & $8.64 \pm 0.18$ & $9.08 \pm 0.14$ \\
M51A & $0.49 \pm 0.02$ & $8.99 \pm 0.08$ & $9.34 \pm 0.06$ & $9.98 \pm 0.06$ & $10.42 \pm 0.05$ \\
M51B & $-1.76 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $9.74 \pm 0.02$ & $10.13 \pm 0.02$ \\
NGC5350 & $0.27 \pm 0.07$ & $8.83 \pm 0.15$ & $9.39 \pm 0.10$ & $10.20 \pm 0.05$ & $10.62 \pm 0.04$ \\
NGC5353 & $-3.73 \pm 4.46$ & $7.73 \pm 0.35$ & $9.76 \pm 0.03$ & $10.66 \pm 0.02$ & $11.03 \pm 0.02$ \\
NGC5354 & $-1.87 \pm 0.08$ & $8.68 \pm 0.07$ & $9.70 \pm 0.02$ & $10.45 \pm 0.02$ & $10.82 \pm 0.02$ \\
NGC5394 & $0.75 \pm 0.03$ & $9.32 \pm 0.27$ & $9.28 \pm 0.09$ & $9.90 \pm 0.03$ & $10.35 \pm 0.02$ \\
NGC5395 & $0.71 \pm 0.05$ & $8.95 \pm 0.10$ & $9.46 \pm 0.07$ & $10.62 \pm 0.04$ & $11.04 \pm 0.03$ \\
NGC5457 & $0.06 \pm 0.02$ & $8.73 \pm 0.23$ & $9.07 \pm 0.09$ & $9.25 \pm 0.04$ & $9.74 \pm 0.03$ \\
NGC5426 & $0.16 \pm 0.42$ & $8.67 \pm 0.49$ & $9.07 \pm 0.34$ & $9.79 \pm 0.17$ & $10.28 \pm 0.11$ \\
NGC5427 & $0.75 \pm 0.19$ & $8.96 \pm 0.43$ & $9.16 \pm 0.25$ & $10.05 \pm 0.12$ & $10.53 \pm 0.08$ \\
NGC5474 & $-2.54 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $7.82 \pm 0.02$ & $8.39 \pm 0.02$ \\
NGC5480 & $0.27 \pm 0.05$ & $9.17 \pm 0.27$ & $9.29 \pm 0.17$ & $9.51 \pm 0.10$ & $9.97 \pm 0.08$ \\
NGC5481 & $-2.87 \pm 1.23$ & $8.14 \pm 0.56$ & $9.66 \pm 0.08$ & $9.94 \pm 0.07$ & $10.32 \pm 0.06$ \\
NGC5544 & $-0.14 \pm 0.02$ & $9.00 \pm 0.02$ & $9.61 \pm 0.02$ & $10.14 \pm 0.02$ & $10.53 \pm 0.02$ \\
NGC5614 & $0.02 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.74 \pm 0.02$ & $11.15 \pm 0.02$ \\
NGC5850 & $-0.16 \pm 0.02$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $10.56 \pm 0.02$ & $10.96 \pm 0.02$ \\
NGC5905 & $0.76 \pm 0.03$ & $9.00 \pm 0.03$ & $9.36 \pm 0.03$ & $10.28 \pm 0.02$ & $10.72 \pm 0.02$ \\
NGC5908 & $0.08 \pm 0.12$ & $8.71 \pm 0.06$ & $9.48 \pm 0.02$ & $10.78 \pm 0.02$ & $11.19 \pm 0.02$ \\
NGC5929 & $-1.03 \pm 0.04$ & $8.70 \pm 0.02$ & $9.48 \pm 0.02$ & $9.69 \pm 0.02$ & $10.10 \pm 0.02$ \\
NGC5930 & $-0.10 \pm 0.33$ & $8.63 \pm 0.37$ & $9.22 \pm 0.31$ & $9.92 \pm 0.21$ & $10.38 \pm 0.15$ \\
NGC5953 & $-0.90 \pm 0.02$ & $7.70 \pm 0.02$ & $8.60 \pm 0.02$ & $9.46 \pm 0.02$ & $10.03 \pm 0.02$ \\
NGC5954 & $0.18 \pm 0.02$ & $9.13 \pm 0.22$ & $9.23 \pm 0.09$ & $9.33 \pm 0.05$ & $9.80 \pm 0.03$ \\
NGC5981 & $-1.67 \pm 0.02$ & $8.70 \pm 0.02$ & $9.60 \pm 0.02$ & $9.83 \pm 0.02$ & $10.22 \pm 0.02$ \\
NGC5985 & $0.36 \pm 0.03$ & $8.94 \pm 0.11$ & $9.55 \pm 0.11$ & $10.56 \pm 0.10$ & $10.96 \pm 0.09$ \\
ARP314A & $0.56 \pm 0.06$ & $9.18 \pm 0.31$ & $9.23 \pm 0.11$ & $9.71 \pm 0.06$ & $10.17 \pm 0.04$ \\
ARP314B & $0.36 \pm 0.02$ & $8.73 \pm 0.18$ & $9.07 \pm 0.07$ & $9.54 \pm 0.03$ & $10.03 \pm 0.02$ \\
NGC7714 & $0.93 \pm 0.02$ & $9.72 \pm 0.16$ & $9.29 \pm 0.06$ & $9.91 \pm 0.06$ & $10.37 \pm 0.05$ \\
NGC7715 & $-1.38 \pm 0.94$ & $7.92 \pm 0.63$ & $8.66 \pm 0.19$ & $8.57 \pm 0.06$ & $9.14 \pm 0.03$ \\
\hline
\end{tabular}

